POW-HOW: An enduring timing side-channel to evade online malware sandboxes

Online malware scanners are one of the best weapons in the arsenal of cybersecurity companies and researchers. A fundamental part of such systems is the sandbox that provides an instrumented and isolated environment (virtualized or emulated) for any user to upload and run unknown artifacts and identify potentially malicious behaviors. The provided API and the wealth of information inthe reports produced by these services have also helped attackers test the efficacy of numerous techniques to make malware hard to detect.The most common technique used by malware for evading the analysis system is to monitor the execution environment, detect the presence of any debugging artifacts, and hide its malicious behavior if needed. This is usually achieved by looking for signals suggesting that the execution environment does not belong to a the native machine, such as specific memory patterns or behavioral traits of certain CPU instructions. In this paper, we show how an attacker can evade detection on such online services by incorporating a Proof-of-Work (PoW) algorithm into a malware sample. Specifically, we leverage the asymptotic behavior of the computational cost of PoW algorithms when they run on some classes of hardware platforms to effectively detect a non bare-metal environment of the malware sandbox analyzer. To prove the validity of this intuition, we design and implement the POW-HOW framework, a tool to automatically implement sandbox detection strategies and embed a test evasion program into an arbitrary malware sample. Our empirical evaluation shows that the proposed evasion technique is durable, hard to fingerprint, and reduces existing malware detection rate by a factor of 10. Moreover, we show how bare-metal environments cannot scale with actual malware submissions rates for consumer services.

==> PoW for VM detection/00_abstract_www.tex <==
\begin{abstract}
Online malware scanners are one of the best weapons in the arsenal of cybersecurity companies and researchers. A fundamental part of such systems is the sandbox that provides an instrumented and isolated environment (virtualized or emulated) for any user to upload and run unknown artifacts and identify potentially malicious behaviors. The provided API and the wealth of information in the reports produced by these services have also helped attackers test the efficacy of numerous techniques to make malware hard to detect. 

The most common technique used by malware for evading the analysis system is to monitor the execution environment, detect the presence of any debugging artifacts, and hide its malicious behavior if needed. This is usually achieved by looking for signals suggesting that the execution environment does not belong to a the native machine, such as specific memory patterns or behavioral traits of certain CPU instructions. 
%To mitigate this threat, sophisticated sandboxes remove or spoof these signals.

In this paper, we show how an attacker can evade detection on such online services by incorporating a Proof-of-Work (PoW) algorithm into a malware sample. Specifically, we leverage the asymptotic behavior of the computational cost of PoW algorithms when they run on some classes of hardware platforms to effectively detect a non bare-metal environment of the malware sandbox analyzer. To prove the validity of this intuition, we design and implement the \name framework, a tool to automatically implement sandbox detection strategies and embed a test evasion program into an arbitrary malware sample. Our empirical evaluation shows that the proposed evasion technique is durable, hard to fingerprint, and reduces existing malware detection rate by a factor of 10.
%making samples not detectable.
Moreover, we show how bare-metal environments cannot scale with actual malware submissions rates for consumer services.
\end{abstract}

==> PoW for VM detection/01_introduction_www.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Malware attacks have a significant financial cost, estimated around \$1.5 trillion dollars annually (or \$2.9 million dollars per minute)~\cite{malwarecost2018}, with predictions hinting at this cost to reach \$6 trillion dollars by 2021~\cite{malwareCost}. Due to the sheer amount of known malware samples~\cite{virushare,virustotalstats},  manual analysis neither scales nor allows to build any comprehensive threat intelligence around the detected cases (\eg malware clustering by specific behavior, family or infection campaign). To address this problem, security researchers have introduced \emph{sandboxes}~\cite{anubis}: isolated environments that automate the dynamic execution of malware and monitor its behavior under different scenarios. Sandboxes usually comprise a set of virtualized or emulated machines, instrumented to gather fundamental information of the malware execution, such as system calls, registry keys accessed or modified, new files created, and memory patterns.

As a next step, online services came to bring malware analysis from security experts to the common users~\cite{sandboxes}. Online malware scanners are not only useful for the users but also for the attackers. In fact by allowing an artefact to be checked multiple times against various state-of-the-art of malware analysis sandboxes, attackers can tune the evasiveness of their malware samples by exploiting the feedback reported by these services and try various techniques before making the sample capable of detecting the presence of a sandbox.
%
Specific CPU instructions, registry keys, memory patterns, and \emph{red pills}~\cite{1624022,fistful,kemufuzzer} are only a few of the signals used by attackers for identifying glitches of the  emulated environment that can disclose the presence of a sandbox environment. These techniques have triggered an arms-race, with the more sophisticated web malware scanners rushing to spoof any such exploitable signals~\cite{barecloud}.

In this work, we show how an attacker can evade malware analysis of these scanning services by leveraging Proof-of-Work (PoW)~\cite{powdwork} algorithms. Our intuition lies on the fact that, like NP-class problems~\cite{npp}, the asymptotic behavior of a PoW algorithm is constant in terms of computational power~\cite{powdwork}, \eg CPU and memory consumption which remain stable over time. Accordingly, PoW algorithms are perfect candidates for benchmarking the computation capability of the underlying hardware. In such scenario the benchmark can be leveraged as a fingerprint of the underlying computing infrastructure, revealing the presence of a sandbox since it shows a statistical deviation compared with the native hardware platform. Moreover, current defensive techniques that aim at spoofing the virtualization signals present in contemporary sandboxes cannot act as countermeasures against the stable timing side-channels that our technique exploits.

A key advantage of using PoW techniques is that they are a time-proof and self-contained mechanism compared to other more fine-grained timing side-channel approaches that try to detect the underlying hardware machine. In fact, our system does not require access to precise timing resources for detecting the emulated environment (\eg network or fine-grained timers). In our evaluation we empirically validate that a PoW-based technique can detect an emulated environment with high precision just by looking at the output of the algorithm (i.e., execution time, and number of successful iterations). Furthermore, %this can be achieved via 
PoW implementations do not raise any suspicion to automated malware sandboxes compared with the stalling code  (\eg infinite loops and/or sleep) that is easier to detect because of CPU idleness~\cite{10.1145/2818000.2818030}. Fingerprinting PoW algorithms as a malware component is feasible \eg by checking the usage of particular cryptographic instructions. However, using it as a proxy signal for detecting malware would produce a large number of false positives since PoW algorithms are part of legitimate applications such as Filecoin ~\cite{filecoin} and Hashcash~\cite{hashcash}.
%compared with more fine-grained ad-hoc side-channel techniques~\cite{10.1145/2818000.2818030}, 

\noindent{\bf Contributions.} %In this paper 
In this paper, we make the following contributions: 
\begin{enumerate}[leftmargin=0.5cm, itemsep=0.2cm]
    \item We design and implement \name: a framework to automatically create, inject, and evaluate PoW-based evasion strategies in arbitrary programs. \name operates as a three-step pipeline. 
    First (step 1) multiple PoW algorithms are thoroughly tested across different hardware platforms (Raspberry Pi 3, Dual Intel Xeon, Intel i9), operating systems (Linux Ubuntu 18.03 and Windows 10), and machine loads. The outcome of these tests (step 2) is used to build a statistical characterization of each PoW's execution time under each setting. We use the Bienaym\'{e}–Chebyshev inequality~\cite{chebychev} to obtain statistical evidence about the expected execution time. Next, a miscreant can upload its malware to the \name framework and select the evasion mechanism to be used. Finally (step 3), \name automatically evaluates the accuracy of the evasion mechanism selected and embedded in the uploaded malware via several tests on multiple online sandbox services~\cite{sandboxes}.
    
    \item We empirically evaluate each step of \name's pipeline. For the PoW threshold estimation, we have tested three popular PoW algorithms
    (Catena~\cite{catena}, Argon2~\cite{argon2,argon2rfc} and Yescrypt~\cite{yescrypt}) using multiple configurations. During 24 hours of testing, we find Chebyshev inequality values higher than 97\% regardless of PoW and setting. This result verifies high determinism in PoW execution times on real hardware, thus validating the main intuition behind this work.  We test our technique on top of two known ransomware families by submitting to three sandboxes several variants that include PoW-based evasion. The results demonstrate how PoW-based evasion %the inclusion of this mechanism 
    reduces the number of detections, even in the presence of anti-analysis techniques such as code virtualization or packing.
    
    \item To further %analyze impact on real-world analysis sandboxes, 
    quantify the efficacy of  PoW-based evasion with real-world sandboxes, we wrote a  fully functional malware sample, integrated with an evasion mechanism based on Argon2, and submitted it to several online sandboxes. All the reports from each sandbox mark our malware as \emph{clean}. %, validating the effectiveness of a PoW-based evasion mechanism. 
    We further discuss the behavioral analysis for our malware, as well as potential countermeasures to this novel PoW-based evasion mechanism we have proposed. To ensure the reproducibility of our results and foster further research on this topic, we make the source code of our system publicly available~\cite{repo}\footnote{ \url{https://github.com/anonnymousubmission/Esorics2021_Paper159}}.
\end{enumerate}

==> PoW for VM detection/02_background.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Background}
\label{sec:background}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Malware and Malware Analysis}
Together with the evolution of malicious software, researchers and professionals have tried to improve their tools and skills to understand malware and counter its consequences. There is a huge amount of literature devoted to analyze and counter malware~\cite{CyberProbe_NDSS14,autoprobe,Gu_ACSAC09_botProber,ppipup,ppi,Wang_Oakland10_TaintScope,DBLP:conf/sp/KolbitschHKK10,DBLP:conf/sp/MoserKK07}. Every aspect of this phenomenon has been taken into consideration, from its network infrastructure, to the code that gets reused among samples, unexplored paths in the control-flow, sandbox design and instrumentation. Nonetheless the arms race keeps running, while new analysis evasion techniques are found, new countermeasures get developed. 

\point{Anti-Analysis Techniques}
There are several anti-analysis techniques which have been developed during the years by miscreants, and promptly countered by our community: \eg packers~\cite{omniunpack,ugarte}, emulators~\cite{rotalume}, anti-debugging and anti-disassembly tricks and stalling code. Among all these techniques the only one that seems to resist is stalling code, which is very difficult to detect~\cite{lastlinestall}. Indeed, over 70\% of all malware attacks involved evasive zero-day malware in Q2 of 2020: a 12\% rise on the previous quarter~\cite{malware2020}. This denotes that evasive malware is a phenomenon that will hardly disappear and there will always be  continuous research in evading analysis systems. 

\subsection{PoW for Malware Analysis Evasion}
Proof-of-Work (PoW)~\cite{powdwork} is a consensus mechanism that imposes computation workload on a node. A key feature of such algorithms is their asymmetry: the work imposed on the node is moderately hard but it is easy for a server to check the computed result. There are two types of PoW protocols: (a) \emph{challenge-response} protocols, which require an % direct 
interactive link between the server and the client, and (b) \emph{solution-verification} protocols, which allow the client to solve a self-imposed problem and send the solution to the server to verify the validity of the problem and its solution. Such %problems 
PoW protocols (also known as CPU cost functions) leverage algorithms like hashcash with doubly iterated SHA256~\cite{laurie2004proof}, momentum birthday collision~\cite{larimer2014momentum}, cuckoo cycle~\cite{tromp2015cuckoo}, and more.

In \name we use Argon2, which guarantees that by using the same input parameters, the amount of computation performed is asymptotically constant; hence, the variance of Argons2's execution time $T$ is very small on the same platform. Moreover, Argon2 is based on a memory-hard function which, even in the case of parallel or specialized execution (\eg ASICs or FPGAs), will not enhance scalability, and hence remains computationally bounded due to its asymptotic behavior. 

The Argon2 algorithm takes the following input:
 \begin{itemize}
     \item A message string $P$, which is a password for password hashing applications. Its length must be within 32-bit size.
     \item A nonce $S$, which is used as salt for password hashing applications. Its length must be within 32-bit size. 
     \item A degree of parallelism $p$ that determines how many independent (but synchronized) threads can be run. Its value should be within 24-bit size (minimum is 1).
     \item A tag, which length should be within 2 and 32-bit. 
     \item A memory size $m$, which is a number expressed in Kibibytes.
     \item A number of internal iterations $t$, which is used to tune the running time independently of the memory size. Its value should be within 32-bit size (minimum is 1).
 \end{itemize}

 These input parameters are used in our framework to define the computational boundary of the algorithm execution on a specific class of hardware machines. Once the parameters are set, the output of the PoW algorithm only depends on the hardware platform. 

\subsection{Side-channel Measurement}
Various techniques have been proposed to detect if applications are running inside a sandbox/virtualizer/emulator. The most reliable of them is based on timing measurements~\cite{timingfoundational}. Indeed, fine grained timers help also to build micro-architectural attacks such as Spectre and Meltdown~\cite{meltdown,spectre}. 
The intuition behind our work is that PoW algorithms offer strong cryptographic properties with a very stable complexity growth, which make the approach very resilient to any countermeasure, such as using more powerful bare-metal machines to enhance performance and reduce the space for time measurements.

By exploiting the asymptotic behavior of the PoW algorithms, we build a statistical model that can be used to guess the class of environment where the algorithm is running and consequently distinguish between physical and virtualized, emulated or simulated architectures, like different flavors of malware sandboxes.
Indeed, even fine grained red-pills techniques~\cite{fistful} such as CPU instruction misbehavior can be easily fixed in the sandbox or spoofed to thwart evasion techniques. On the other hand PoW stands on top of well defined mathematical and well defined computational behavior. Moreover, a simple modification of the PoW library avoids the malware sample to be fingerprinted by static techniques. If we take as an example of PoW complexity the one that is run in the crypto currency environment, we know that by design the computation complexity of the algorithm is increased for each new block of the blockchain transaction~\cite{bitcoin}. Such an increase of computation shows the asymptotic behavior that can be exploited by our technique. By applying PoW as a malware sandbox evasion technique, we get an off-the-shelf technique which improves the malware resilience and limits its analysis. 

==> PoW for VM detection/03_approach.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Our Approach: \name}
\label{sec:framework}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This section describes our threat model before describing our approach in detail. We first provide an overview of the technique (Section~\ref{sec:framework:overview}) and its main workflow. We then describe how the key parameters are estimated (Sections~\ref{sec:framework:measurem} and \ref{sec:framework:estim}) and how an arbitrary sample can be equipped with the evasion module (Section~\ref{sec:framework:integration}).

\subsection{Threat Model}
\label{sec:threat}
In this paper, we assume a malware scanning service based on virtualized or emulated sandboxes, which allows users to upload and scan their individual files for free as many times as they need. Such a service joins together results from various state-of-the-art malware analysis sandboxes before responding back to the user with a detailed report about the detection outcome of each and every sandbox scanner used.  

On the other hand, we assume an attacker who developed a program that includes (i) some malicious payload along with (ii) a technique to pause or alter the execution of the malicious program itself, when a possible malware analysis environment is detected. Before distributing the malicious program to the victims, the attacker may use a malware scanning service to assess its evasiveness.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{System Design}
\label{sec:framework:overview}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
As described in Section~\ref{sec:background}, PoW puzzles have moderately high solving cost and a very small verification time, like problems in the NP complexity class~\cite{npp}. This implies that their asymptotic behavior is constant in terms of computational cost~\cite{powdwork}, \eg CPU and memory consumption. \name exploits this asymptotic behavior to build a statistical model that can be used to identify the class of hardware machines where the algorithm is running. Such a model can later be used to distinguish between physical and virtualized architectures, like those present in  malware sandboxes. \name is a three-step pipeline (see Figure~\ref{fig:arch}):
\begin{enumerate}
    \item \textit{Performance Profiling}. It %first 
    executes multiple PoW algorithms on several hardware %platforms 
    and operating systems using different configuration settings and system loads.
    \item \textit{Model estimation}. The previous step provides the system with a measurement of the amount of time needed to execute the PoW on real hardware. By using the Bienaym\'{e}–Chebyshev~\cite{chebychev} inequality, it then estimates the time (threshold) expected for a particular configuration to run on a given architecture.
    \item \textit{Integration}. Once the models are built, a malware developer can select a specific PoW and parameters to associate with an arbitrary malware sample. \name then generates a module with the chosen PoW, which is integrated with the sample by building a single statically-linked executable.
\end{enumerate}
As ground truth, our methodology leverages a custom Cuckoo Sandbox~\cite{cuckoo} and  popular crowd-sourced malware scanning services (like VirusTotal or similar~\cite{sandboxes}), as a testbed to report on the accuracy of the evasiveness of the malware in real-world settings.

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figs/arch.pdf}
    \caption{High level overview of \name. Step 1: execution of the PoW 
    on several hardware/OSes using different configuration settings and system load. Step 2: threshold estimation based on execution time per configuration/architecture. Step 3: malware integration and test.}
\label{fig:arch}\vspace{-0.4cm}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Performance Profiling}
\label{sec:framework:measurem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The first step in \name's pipeline produces a number of PoW executions using different algorithms, parameters, hardware, operating systems, and load settings:

\point{Hardware}
\name leverages three machines representative of low, medium, and high-end platforms. The high-end machine is a desktop equipped with an Intel(R) Core(TM) i9-9900X CPU @ 3.50GHz with 10 physical cores and 20 threads equipped with a PCI-e M2 512GB disk and 32 GB of RAM. The medium-end machine is a workstation equipped with a Dual Intel(R) Xeon(R) CPU E5-2643 0 @ 3.30GHz with 16 physical cores and 64GB of RAM. Finally, the low-end device is a \rpi which comes with a quad core ARMv7 Processor rev 4 (v7l) and 1GB of RAM.

\point{Systems and loads}
With the exception of the \rpi, the other hardware platforms are setup in dual boot, supporting both Linux Ubuntu 18.04.3 (64 bits) and Windows 10 (64 bits). Each platform can be further configured in \emph{idle} and \emph{busy} mode. The latter is achieved using \texttt{iperf}~\cite{perf} a CPU bound network traffic generator to keep the operating system and the CPU occupied. 

\point{PoW and parameters}
\name currently supports three popular PoW algorithms: Catena~\cite{catena}, Argon2~\cite{argon2,argon2rfc}, and Yescrypt~\cite{yescrypt}.
Each PoW algorithm is executed multiple times with different input parameters on each hardware platform, operating system, and load setting. The parameters of each algorithm allow to control the amount of memory, parallelism, and complexity of the PoW. Our selection is based on common configuration of COTS hardware devices, with respect to memory and CPU. However, not all the selected algorithms have these parameters available for tuning and in some cases, their tuning is more coarse grained~\cite{catena}. 


\subsection{Threshold Estimation}
\label{sec:framework:estim}
The second step in \name's pipeline aims at estimating the PoW thresholds for different settings (PoW algorithm, parameters, hardware, operating system, and load). This is achieved through a statistical characterization of the execution time in each setting using the Bienaym\'{e}–Chebyshev inequality~\cite{chebychev}. This is a well-known result in probability theory stating that for a large class of distributions, no more than $\frac{1}{k^2}$ values of a distribution $X$ can be more than $k$ standard deviations ($\sigma$) away from the mean ($\mu$):

\begin{equation}
Pr(|X - \mu| \geq k\sigma) \leq \frac{1}{k^2}
\end{equation}

Using the empirical distribution of execution time observed in the previous step, this inequality allows us to select a threshold $T$ (\ie a maximum execution time) which guarantees a high sample population coverage. The previous deduction enables us to determine with high probability the time $T$ it will take for a PoW to run if the underlying platform is not virtualized. To reduce false positives, the evasion rule can be generalized to ``the execution environment is virtualized if the PoW does not complete $N$ executions in less than $T$ seconds.''


\subsection{Malware Integration and Testing}
\label{sec:framework:integration}
The final step in \name's pipeline is PoW integration with a malware sample provided as input. At this step, the attacker can upload its sample to \name and select the PoW-based evasion mechanism to be used,  along with its parameters. \name further informs the attacker about the predicted accuracy of this selection.

\name integrates the uploaded malware with the PoW selected and the Boost C++ libraries~\cite{boost}, which ease the OS interaction to build a single statically-linked executable. The compilation stage is automated as an Ansible~\cite{ansible} playbook and clang~\cite{clang}. The integration is achieved at linking stage, so the malware will have a stub call to an external symbol that will be linked with the chosen PoW. \name's pipeline then starts the Ansible scripts, which runs some tests and launch the compilation of the final binary for multiple platforms automatically.

\point{Testing}
To evaluate the accuracy of the newly generated evasion mechanism, we rely both on a local sandbox---a custom Cuckoo Sandbox~\cite{cuckoo} equipped with Windows 10 (64 bits), which is the most targeted OS for malware campaigns~\cite{wannacry}---and several on-line free-of-charge sandbox services~\cite{sandboxes}. Once this step is completed, \name offers to the user access to the set of reports generated by each sandbox.


==> PoW for VM detection/04_evaluation.tex <==
\section{Evaluation}
\label{sec:eval}

In this section, we evaluate \name's pipeline. We first analyze the combination of PoWs and their parameters currently supported by \name. The outcome of this evaluation are the parameters $N$ (cycle of execution made in less than $T$ second) and $T$ (maximum execution time) to be associated with the malware sample. We then discuss the accuracy of our evasion mechanism across using various case studies across three public malware scanning services: (~\cite{joesandbox}, ~\cite{hanalysis},~\cite{virustotal}), along with our own Cuckoo Sandbox instance. 

\begin{table}[t]
\centering
\makebox[0pt][c]{\parbox{\textwidth}{%
    \begin{minipage}[t]{0.48\textwidth}
\centering
\scriptsize
    \begin{tabular}{lrrrr}
    \toprule 
        \bf Platform  & \bf Status &  \bf Win 10 & \bf Ubuntu 18.03  \\
    %&&& \bf Ubuntu 18.03 \\
        \midrule
        Intel i9 & \emph{idle}   & 4,500 & 9,325 \\
        & \emph{busy}            & 3,642 & 8,867\\ 
        \midrule
        Dual Intel Xeon & \emph{idle} & 6,005 & 7,897\\
        & \emph{busy}            &    4,320 & 7,012\\ 
        \midrule
        \rpi   & \emph{idle}     &     -  & 300\\
        & \emph{busy}            &     -  & 143 \\
    \bottomrule
    \end{tabular}
    \caption{Number of consecutive PoW executions per hardware and OS combination over 24 hours. For a given platform, the first line refers to results obtained with the \emph{idle} setting, while the second line refers to \emph{busy} setting.}
    \label{tab:hw_totals1}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth}
    \centering
    \scriptsize
    \begin{tabular}{lrrrrrr}
    \toprule
    \bf Garlic Graph Size   & \bf Min & \bf Max & \bf Sigma & \bf Mean & \bf K &\bf Chebyshev \\
     \midrule
    15 & 0.12 & 5.35 &   0.503 &  0.209 & 9.99 &          99.00\% \\
    18 & 1.13 & 35.61 &   4.22 &  1.86 & 7.94 &          98.41\% \\
    20 & 5.11 & 165.57 &  19.01 &  8.26 & 8.26 &          98.54\% \\
    \bottomrule
    \end{tabular}
    \caption{Statistical measurement results for Catena.}
    \label{tab:catena}
\end{minipage}
}}\vspace{-0.5cm}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Threshold Estimation and PoW Algorithm Choice}
\label{lab:estimation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% currently supported by \name, 
For each PoW, we have selected different configurations with respect to memory footprint, parallelism, and algorithm internal iterations (see Tables~\ref{tab:catena} for Catena and ~\ref{tab:argon-yescrypt} for Argon2i and Yescryot). Argon2i and Yescrypt have similar parameters (memory, number of threads, blocks) whereas Catena's only parameter is a graph size which grows in memory and will make its computation harder as the graph size increases.

\name executes each PoW configuration on the low-end (\rpi), medium-end (Dual Intel Xeon), and high-end (Intel i9) machines. All PoW configurations are executed sequentially during 24 hours on each machine for both idle and busy conditions. As pointed out in Section~\ref{sec:framework}, with the exception of the \rpi, all tests are performed on two operating system per hardware platform: Linux Ubuntu 18.04.3 (64 bits) and Windows 10 (64 bits). 


Table~\ref{tab:hw_totals1} shows the total number of PoW executed over 24 hours per hardware, operating systems, and CPU load (\emph{idle} or \emph{busy}). Regardless of the CPU load on each machine, we observe two key insights. First, there is a significant drop in the number of PoW executions when considering Linux vs Windows, which is close to a 50\% reduction in the high-end machine. This is due %, to the best of our knowledge, 
to operating system interaction, ABI and binary format, and ultimately idle cycle management. Second, a 30x reduction in the number of PoW executions when comparing high-end and low-end platforms, \eg under no additional load the \rpi completes 300 executions versus an average of 8,611 executions on both the high and medium-end machines. Finally, extra load on the medium and high-end machines  causes a reduction in number of proofs computation of about 6-10\%, averaging out to 7,300 executions between the two machines. A more dramatic 50\% reduction was instead measured for the \rpi. 


Next, we statistically investigate PoW execution times by mean of the Bienaym\'{e}–Chebyshev inequality (see Section~\ref{sec:framework:estim}). To balance equally sized datasets, we sampled 150 random executions (\ie the total number of executions that were possible to complete on the low-end platform) from the 9,325 executions available from both the medium and high-end platforms.  
Tables~\ref{tab:catena} and~\ref{tab:argon-yescrypt} show for each PoW and configuration, several statistics (min, max, $\sigma$, and $K$, Chebyshev inequality) of the PoW execution time computed across hardware platforms, OSes (when available), and load condition (idle, busy). Overall, we measured Chebyshev inequality values higher than 97\% regardless of the PoW and its configuration. This confirms high determinism in the PoW execution times on real hardware, validating the main intuition behind this work. 

\point{Algorithm choice}
The results above provide the basis to select a PoW algorithm along with its parameters to integrate with the input malware sample. These results indicate  that PoW selection has minimal impact on the expected accuracy of the proposed evasion mechanism. We then selected Argon2i (with 8 threads, 100 internal functions and 4KiB of memory) motivated by its robustness and maturity.
% we do not exclude to involve new generation of Catena and Yescrypt.
%\name to automatically integrate the PoW with our PoC ransomware~\cite{ransomware}. it selected its parameters to be close to an average COTS PC. 
We leverage the results from Table~\ref{tab:argon-yescrypt} (top, second line) to set the parameters $N$ (PoW execution) and $T$ (evasion threshold) of an  Argon-based evasion mechanism. The table shows that $K=8.1$ seconds allows a good coverage for the execution time population (98.3\%). We  opted for a more conservative value of $T=10$ and further performed  multiple tests on our internal Cuckoo Sandbox. Given that our Cuckoo Sandbox could not even execute 1 PoW with $T=10$, we simply set $N>1$. We will use this configuration for the experimentation described in the remaining of this paper.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\point{Evasion Accuracy Estimation}
\subsection{Case Study: Known Malware}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We first analyze the effect of adding our PoW-based evasion strategy to the code of two well-known ransomware samples: Relec and Forbidden Tear.  The use of real-world malwares, which are well know and thus easy to detect, allows us to comment on the impact that PoW-based evasion has on \textit{malware reuse}, the practice of recycling old malware for new attacks. We use \name to generate various combinations of each original ransomware with/without PoW-based evasion strategy, code virtualization\footnote{This cannot be applied to ForbiddenTear since it is written in .NET.}, and packing offered by Themida, a well-known commercial packer~\cite{themida}. We verify that all the malicious operations of the original malwares were preserved across the generated versions. 

\begin{table}[t]
\centering
\makebox[0pt][c]{\parbox{\textwidth}{%
    \begin{minipage}[t]{0.48\textwidth}    \centering
    \scriptsize
    \begin{tabular}{lrrrrrrrr}
    \toprule
     \bf Thr. & \bf It. & \bf Mem. & \bf Min & \bf Max & \bf Sigma & \bf Mean & \bf K & \bf Cheb.\\
    \midrule
     1 & 10   & 1KB  & 0.01 & 0.70 &  0.09 &  0.02 & 7.9 & 98.4\% \\
     8 & 100  & 4KB  & 0.20 & 9.28 &  1.07 & 0.46 & 8.1 & 98.3\% \\ 
     16 & 500 & 8KB  &  2.03 & 88.8 &  10.5 &  3.85 & 7.9 & 98.4\% \\
    \midrule
    \midrule
    1 & 1K    & 8KB  & 0.00 & 0.02 &   0.00 &  0.01 & 6.1 &  97.3\% \\
    8 & 2K    & 32KB & 0.03 & 0.56 &   0.05 &  0.05 & 10.5 & 99.1\% \\
    16 & 4K   & 64KB & 0.08 & 5.00 &   0.51 &  0.19 & 9.4 & 98.9\% \\
    \bottomrule
    \end{tabular}
    \caption{Statistical measurement results for Argon2i (top) and Yescrypt (bottom). Thr. = number of threads. It. = number of algorithm steps. Mem. = amount of memory used in KiB. Cheb. = Chebyshev coverage.}
    \label{tab:argon-yescrypt}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth}    \centering
    \centering
    \scriptsize
    \begin{tabular}{lrrr}
    \toprule
      \bf Test & \bf Relec & \bf Forbidden  & \bf Hello \\
      & & \bf Tear & \bf World \\
        \midrule
        Original                    & 23/72   & 26/72  & 3/72\\ 
        \begin{tabular}{@{}l@{}}Original+Code Virtualizer\end{tabular}& 32/72   & n/a   & 19/72 \\
        Original+Themida            & 33/72   & 21/72  & 17/72 \\
        \begin{tabular}{@{}l@{}}Original+PoW+Code Virtualizer\end{tabular} & 29/72   & n/a   & 0/72 \\ 
        Original+PoW+Themida        & 32/72   & 18/72  & 9/72 \\ 
        \bf Original+PoW                & \bf 3/71   & \bf 3/72  & \bf 2/72  \\ 
    \bottomrule
    \end{tabular}
    \caption{Online Sandbox detection results for 2 ransomware samples (Relec and Forbidden Tear) and a benign test program using various anti-analysis configurations.}
    \label{tab:caseStudies}
    \end{minipage}
    }}\vspace{-0.5cm}
\end{table}

We submitted all malware variants to three online sandboxes for analysis and checked how many AV engines (antivirus products) flag each variant as malicious (see Table~\ref{tab:caseStudies}). In the case of Relec, adding code virtualization or packing, results in more AV engines detecting the sample as malicious. This is likely due to the engines flagging such protections, not the malware sample itself. In all cases, the addition of PoW decreases the number of detections by a factor of 10~\cite{vtrelecnostrings}, reaching a level where the difference between the label \textit{malicious} and \textit{false positive} is evanescent. 

Table~\ref{tab:caseStudies} also show results when submitting several variants of a standard Hello World program. Note that the original code has been flagged as malicious by 3 AV engines, though as it is possible to see from the report the detections are mislabeled \ie{ Relec is not recognized}. This false positive could be due to a large number of submissions of the same code hash (due to its simplicity and popularity), our source IP being flagged, and other unknown factors which may influence the scoring. The table also shows that adding code virtualization or packing translates into a substantial increase in false positive detections even of a simple Hello World program, confirming our intuition above. Instead, adding our PoW-based evasion strategy results in less false positives, one less than the original code. This is likely due to the fact that our code on top of Hello World has more entropy, respect to a very simple one line program, looking more legit to engines that measure such kind of parameters.

Overall, these three case studies show that a PoW-based evasion strategy reduces the number of detections by 10x with known malware by preventing the sample from executing in the analysis sandbox. This result demonstrates large potential for malware reuse by coupling it with PoW-based evasion strategy. In the next section, we perform more controlled experiments based on \textit{fresh} (\ie previously unseen) malware.

\begin{figure}[t]
    \centering
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\columnwidth]{figs/malware1.pdf}
        \caption{Behavioral map of the malware PoC \emph{without} PoW and \emph{without} full static protection enabled.}
        \label{fig:nostrip}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\columnwidth]{figs/malware2.pdf}
        \caption{Behavioral map of the malware PoC  \emph{without} PoW and \emph{with} full static protection enabled.}
        \label{fig:evader}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\columnwidth]{figs/malware3.pdf}
        \caption{Behavioral map of the malware PoC  \emph{with} PoW and \emph{with} full static protection enabled.}
        \label{fig:naked}
    \end{minipage}\vspace{-0.4cm}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Case Study: Fresh Malware Sample}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In order to further explore the results obtained in the previous case studies, we wrote a simple malware PoC (roughly~150 LoC) for Windows 10 (VC++) and Linux (C++). Our malware sample implements a basic ransomware functionality which scans the entire hard drive and encrypts all its files. This behavior should be easy to detect by any malware scanning services.\footnote{The malware detection report for this malware without our PoW-based evasive measure has been anonymized~\cite{noteva,mal_vt}.} Using \name, we automatically embed a PoW (Argon2i, as we will discuss below) and make sure to exhibit its malicious activity only if the PoW is successfully executed at least $N$ times before a timeout $T$. 
Finally, we submitted different variants of our malware sample (with PoW, without PoW, with static sanitization) %and their combinations 
to several on-line sandboxes and the results were disheartening (see Table~\ref{tab:malsand}). For the static sanitation we remove the symbol tables and debugging symbols. Note that very similar results were also achieved with our local Cuckoo Sandbox.
It is important to note that to check the execution of the malware payload
we insert a \emph{create-file} function at the beginning of the malware payload
itself. Such file creation is visible on the behavioral report of the
analyzed sandboxes in case the malware payload is executed\footnote{This reference has been anonymized not to violate the terms of service of sandbox vendors~\cite{noteva}}. We used such a simple test to check whether the PoW algorithm detects
the emulated environment and so validate our technique. In case such a file is not present on the
behavioral report, it means the PoW algorithm detects the emulated environment and
stops the payload execution.
None of the analyzed sandboxes is able to execute more than 1 PoW during $T=10$ (or even $T=20$ sec), which is worse than what a \rpi can do even in presence of some extra load (\eg see max value in the top of Table~\ref{tab:hw_totals1}).


We made all the reports of our analysis publicly available, including screenshots of evasive malware samples~\footnote{The references have been anonymized not to violate the terms of service of sandbox vendors~\cite{eva1,eva2,eva3,eva4,eva5,evavt,evavtsgamo}}. It has to be noted that not all sandboxes report are the same, but they all signal the hard drive scan (Ransomware behavior) without full static protection (i.e., with the default compiler options). In Table~\ref{tab:malsand} the number of PoW executed is visible only if a screenshot of the sandbox is available. As for the sandbox execution timeout, not all the analysis services had it available for selection.

\point{Detection Rate Decrease}
As it is possible to see \name's approach is capable of reducing to zero the detection rate of roughly 70 antiviruses run by the tested sandboxes~\cite{virustotal,joesandbox,hanalysis} for any sample that we have tested. We have investigated the multiple facets of our technique (static and dynamic). Thus we conclude after looking also at the behavioural results of our samples that the whole technique is capable of reducing the detection rate to zero. The behavioural part plays a fundamental role as it is possible to see from the Hello World example and the behavioural maps generated by AV labels of Figures~\ref{fig:nostrip}-\ref{fig:naked}.

==> PoW for VM detection/05_sec_analysis.tex <==


%**********************************************************************
% These are the old behavioral maps in three separate figures
%**********************************************************************

%\begin{figure*}[t]
%    \begin{tabular}{ccc}
%    \includegraphics[width=0.64\columnwidth]{figs/evader_nostrip.png} &
%    \includegraphics[width=0.65\columnwidth]{figs/evader.png} &
%    \includegraphics[width=0.72\columnwidth]{figs/strip_nopow.png}\\
%    (a) No PoW and no static protection &
%    (b) No PoW and full static protection &
%    (c) PoW and and full static protection\\
%    \end{tabular}
%    \caption{Behavioral maps of a malware PoC with various combinations of PoW and static protection.}\label{fig:behavioralMaps}
%\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Security Analysis}
\label{sec:analysis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The results shown in the previous section demonstrate that a \name-ed malware can effectively detect a sandbox and abort the execution of any malicious payload. This strategy is effective in getting a malware sample marked as ``clean'' by all sandboxes tested by \name (see Table~\ref{tab:malsand}). \textbf{\name's technique is simple to deploy, it does not require precise timing measurements and, thanks to its algorithmic properties, it will last for many years as a potential threat.}

We next discuss in detail the \emph{behavioral} analysis of our malware. This is an analysis produced by a sandbox related to how a malware interacts with file system, network, and memory. If any of the monitored operations matches a known pattern, the sandbox can raise an alarm.  

\begin{table}[t]
\centering
\scriptsize
    \begin{tabular}{lrrrrr}
    \toprule
    \bf Sandbox & \bf Evasion Timeout & \bf PoW  Timeout &\bf \# of PoW executed & \bf Timeout  & \bf Notes \\
    \midrule
    Sandbox1 & $10$ secs & 50 & 1 & 120 & Clean\\
    Sandbox1 & $15$ secs & 45 & 1 & 180 & Clean\\
    Sandbox1 & $20$ secs & 40 & 1 & 240 & Clean\\
    Sandbox1 & $20$ secs & 15 & 1 & 500 & Clean\\
    Sandbox2 & $20$ secs & 15 & 0 & N/A & Clean\\
    Sandbox3 & $20$ secs & 45 & N/A & N/A & Clean\\
    Sandbox3 & $20$ secs & 15 & N/A & N/A & Clean\\
    \bottomrule
    \end{tabular}
    \caption{Execution results of a custom ransomware sample on various sandboxes}
    \label{tab:malsand}\vspace{-0.6cm}
\end{table}

Figures~\ref{fig:nostrip},~\ref{fig:evader}, and~\ref{fig:naked} show the behavioral analysis of our malware on a radar plot, labelled with most prevalent AV labels. The samples were submitted with different combinations of PoW and static protection. In Figure~\ref{fig:nostrip}, the radar plot is mostly ``green'' (benign) with respect to some operations like phishing, banker and adware for which we would not expect otherwise. However, four ``suspicious'' (orange) behaviors are reported with respect to evader, spyware, ransomware, Trojan operations. While our malware PoC is not labeled as ``malicious'' (red), the suspicious flags for our binary would trigger further manual analysis that coukd reveal its  maliciousness. It is thus paramount to investigate and mitigate such suspicious flags. 

Our intuition is that the suspicious flags are due to the fact that our malware is neither packed nor stripped, and hence some of its functionality \ie exported functions, linked libraries, and function names are visible through basic static analysis that is usually also implemented in the dynamic sandbox environment. %Such information can be used to infer whether the unknown program is implementing suspicious activities.
Accordingly, we strip out the  whole static information from our binary and resubmit it as a new binary. Figure~\ref{fig:evader} shows the behavioral analysis of our PoC malware without PoW-based sandbox detection but with full static protection enabled. As expected, various signals have dropped from the behavioral report. Finally, Figure~\ref{fig:naked} shows the result of adding PoW to the last binary. A completely green radar plot which does not raise any suspicion illustrates the evasion effect of \name. 

\begin{figure}[t]
\centering
\begin{minipage}[t]{0.32\textwidth}
\centering
    \includegraphics[width=1\columnwidth]{figs/cpu_evader.pdf}
    \caption{CPU consumption  of our malware PoC (Argon2d) Malware:red line, System Idle (PID 0):green line.}
    \label{fig:cpueva}
\end{minipage}
\hfill
\begin{minipage}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=1\columnwidth]{figs/evader_mem.pdf}
    \caption{Memory consumption  of our malware PoC (Argon2d) Malware:red line, System Idle (PID 0):green line.}
    \label{fig:mem_footprint}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=1\columnwidth]{figs/evader_ant2.pdf}
    \caption{CPU consumption of our malware PoC. T=60 seconds and 0.5 seconds between each PoW execution. Malware:red line, System Idle (PID 0):green line.}
    \label{fig:evader_ant2}
    \end{minipage}\vspace{-0.4cm}
\end{figure}


%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.73\columnwidth]{figs/evader_nostrip.png}
%    \caption{Behavioral map of the malware PoC \emph{without} PoW and \emph{without} full static protection enabled.}
%    \label{fig:nostrip}
%\end{figure}


%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.73\columnwidth]{figs/evader.png}
%    \caption{Behavioral map of the malware PoC  \emph{without} PoW and \emph{with} full static protection enabled.}
%    \label{fig:evader}
%\end{figure}

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.73\columnwidth]{figs/strip_nopow.png}
%    \caption{Behavioral map of the malware PoC  \emph{with} PoW and \emph{with} full static protection enabled.}
%    \label{fig:naked}
%\end{figure}


\point{CPU and memory usage}
The main downside of associating a PoW with a malware sample is an increase in both CPU and memory consumption.  We here report on CPU and memory consumption as measured by our sandbox. 
Figures~\ref{fig:cpueva} and~\ref{fig:mem_footprint}  compare, respectively, CPU and memory utilization of our malware (red line) with System Idle (PID 0). With respect to  CPU usage, the PoW associated with our malware causes an (expected) 100\% utilization for the whole duration of the PoW ($T=10$~sec). With respect to  memory utilization, our malware only requires about 17~MB versus the 7~MB that utilizes a sample system process like System Idle (PID 0). This is a minor increase, unlikely to raise any suspicion. 

% Next, we investigate whether we can reduce the CPU usage of our PoC ransomware. First we have reduced the PoW execution and the timeout $T$ to 3 seconds and obtained less CPU drain, with a peak of 80\% (see Figure~\ref{fig:evader_ant}). The complete report is available here~\cite{mal_ant1}. This reduces the suspiciousness of our malware as well as the margin error in sandbox detection.  %However, using such a small $T$ (3 seconds) reduces also the margin to evade the sandbox and hence easily detectable.


Next, we investigate whether we can reduce the CPU usage of our PoC ransomware
%An alternative approach consist in making our PoW go ``low-and-slow'', 
by setting a longer $T$ (\eg 60~sec) and a sleep of $0.5$~sec between each PoW execution. Despite such sleeps, Figure~\ref{fig:evader_ant2} still shows 100\%  CPU utilization for the whole $T$ (60~sec in this test). The lack of CPU reduction associated with the extra sleeps is counter-intuitive. The likely explanation is that the  sandbox leverages a coarse CPU monitoring tool and, thus, the CPU reduction associated with our extra sleeps gets averaged out. %It follows that to hide the PoW extra CPU utilization, we would have to further increase the sleep duration effectively transforming our approach into a stalling code solution. Nevertheless, even this ``low-and-slow'' variation of our evasion scheme still goes undetected, as we can observe in the report from Joe's sandbox~\cite{mal_ant2}. 
%
These results provide a foundation to detect evasion techniques based on PoW. A sandbox could %adopt %use an agnostic technique that does not depend on the OS interactions. In particular they should detect the side-channel activities by 
attempt heuristics based on a binary's CPU and memory consumption. We argue, however, that this is quite challenging because of the potential high number of false positives that can be generated.

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.6\columnwidth]{figs/evader_ant2.pdf}
%    \caption{CPU consumption of our malware PoC. T=60 seconds and 0.5 seconds between each PoW execution. Malware:red line, System Idle (PID 0):green line.}
%    \label{fig:evader_ant2}
%\end{figure}

==> PoW for VM detection/06_countermeasures.tex <==
\section{Countermeasures}
\label{sec:defences}

Evasion techniques are easily comparable with other anti-analysis techniques like \emph{packing}. Packing techniques have evolved to such sophistication that it has become practically impossible to unpack a malware sample without dynamically executing it~\cite{lineage,ugarte}. However, dynamically executing a sample can indeed trigger evasion techniques like stalling code. To counter evasion techniques, and especially the ones that \name implements, one idea would be to fingerprint the algorithms, \eg CPU and memory footprint. However, it would be very easy for attackers to apply code polimorphism techniques and produce variants that diverge from the original implementation, as it is done with packers. This will constitute a challenge for the sandbox, which could generate a false negative by not being able to spot the algorithm. In Table~\ref{tab:caseStudies},  the Hello World program is detected as malicious and our technique reduces its detection rate and with a code virtualizer it makes the sample completely stealth. 

\point{Fingerprinting evasion}
A common solution against red pills~\cite{fistful} is to reduce the amount of instructions failing due to emulation. As Martignoni et al.~\cite{emufuzzer,kemufuzzer} show, the analysis can be automated and the fixes can be easily produced. However, with PoW the computational model is not seeking for emulation/virtualization failures or malfunctions. Instead, PoW is acting as a probe to spot a side channel in the execution time of the algorithm, which in this case is time-based.

\point{Virtualized instructions set} Native execution of the cryptographic instructions is another potential countermeasure that could be considered to mitigate our approach.
In such a case, the cryptographic instructions of the PoW algorithm are not emulated by the sandbox environment, but directly executed on the native CPU. Avoiding the emulation of the cryptographic instructions could clearly improve the computational performance of the PoW algorithm and reduce the success probability of the evasive behavior showed by \name.
%
The technique described in the Inspector Gadget paper~\cite{DBLP:conf/sp/KolbitschHKK10}, which works at the program analysis level, may also work to avoid the execution of our evasion code. Once the sample is unpacked, it would be possible to extract and execute only the malware branch of the code as a gadget and analyze its behavior in isolation. However, a sufficiently complex packer or emulator would make such process very tedious and require manual effort, which makes this solution excessively complex to be implemented in an automated malware analysis service.

\point{Specialized hardware}
Even if our choice, Argon2, is resilient to specialized circuits for mining (ASICs and FPGAs), other PoW algorithms are not, and hence an analyst could equip his sandbox with a miner~\cite{antminer}. Such a dedicated hardware is expensive for a non-professional user (around $\$3,000$ at the time of writing). Nonetheless, if the phenomenon of sandbox evasion due to PoW proliferate, having such a platform would be of great help to offload the PoW calculations, through a tailored interface, and continue the execution of the malware sample inside the sandbox. The cost/benefit trade-off of adopting such a measure really depends on the intended scale of the analysis platform. For example, according to VirusTotal statistics~\cite{virustotalstats}, the service receives weekly more than 3M PE binaries. Hence, a dedicated hardware to defeat PoW evasion based techniques  seem a good compromise, since it allows to analyze and discover new malicious behaviors.

\point{Spoofing timers}
The sandbox that gets a \name-ed malware could try to delay the time, which could mean to make our $T=10$ seconds last much longer to achieve the payload execution. This approach may work well. Though, if we expect a total of at least 50 PoW iterations (see Section~\ref{sec:framework:estim}) and the sandbox is not able to execute more than one in about a minute for a unique malware sample, the analysis would take more than one hour. This will eventually extract the payload that will then require extra work to be reverse engineered, understood, and fingerprinted. Hence, this approach may not scale in terms of time/cost for the large number of samples that online sandboxes analyze daily.

\point{Bare-Metal Sandboxes} Using bare metal hardware represents a reasonable solution that might be adopted within corporate companies but it is not possible to use such technology at Internet scale, \ie cloud-based solutions like Virus Total. Also, isolated sandboxes do not benefit of the information that on-line in cloud services have which leverages large scale cross-correlations.

==> PoW for VM detection/07_discussion.tex <==
\section{Discussion}

\subsection{Ethical Considerations}
\label{sec:ethics}
The results obtained by \name regarding the analyzed publicly available sandboxes, normally used by malware analysts under their term of service (ToS), demonstrate that our technique works consistently either in our custom Cuckoo Sandbox implementation or in proprietary solutions. Our aim, though, is not to disrupt any business nor to difficult the operation of companies that profit from providing malware behavior analysis. We contacted all the platforms and vendors that we have tested with \name and we notified them about our findings. Part of the vendors were very positive and agreed to further collaborate to work on practical countermeasures. %But, unfortunately some others seemed more conservative, 
Unfortunately, the response we received from other vendors opposed any dissemination of our results, adopting a shortsighted security-through-obscurity approach which is not novel in our community.
Consequently, tested vendors have been anonymized to avoid violation of their ToS. We purposely maintained the number of new variants submitted to the bare minimum, but our approach may transform easily any existing sample into a new one. The authors are available for contact for further information disclosure.

\subsection{Bare-Metal Environments}
In~\cite{barecloud} the authors present BareCloud a bare-metal system which helps to detect evasive malware. This system in order to execute malware trades visibility against transparency. In other words it makes the analysis system transparent (non-detectable by malware) and produces less powerful analysis data (limited instrumentation). Indeed their detection technique leverages hierarchical similarity~\cite{kdd} comparison between different malware execution traces (virtualized and emulated) systems i.e., (Ether~\cite{ether}, Anubis~\cite{anubis}, and VirtualBox~\cite{cuckoo}). One of the biggest problem of hierarchical similarity algorithms is scalability, which means that the algorithm should be polynomial in time and space. An example~\cite{simil} of application and analysis of hierarchical similarity for binary program comparison shows $O(n^2)$ complexity. Hence using BareCloud as a production system for example for VirusTotal which claims~\cite{virustotalstats} about 1.5M daily submissions means that the hierarchical comparison would approximate 2.250 billion of operations daily to detect evasive malware with bare metal equipment. It is evident that BareCloud can be useful in special cases, as briefly stated above, where also a manual analyst can make the difference. For the sake of scalability though virtualization and emulation methods cannot be fully replaced, even if it would be possible to instrument in hardware an entire system~\cite{10.1145/2818000.2818030}, the approach would suffer many other issues, for instance having a lot of physical hardware and maintaining it.
%
%\point{Evasive malware on the rise} Over 70\% of all malware attacks involved evasive zero-day malware in Q2 of 2020: a 12\% rise on the previous quarter~\cite{malware2020}. This denotes that evasive malware is a phenomenon that will hardly disappear and there will always be  continuous research in evading analysis systems. 
%
%Recently, a well-known sandbox vendor declared that ``detecting evasive samples is not a priority for their business'' (via private communication). While this statement suggests that online services might not pay special attention, if samples try to evade their aggregated detection system, this does not imply that such evasion is going to disappear. This statement, though, may open avenues for a different attack surface, such as Economical Denial of Sustainability~\cite{edos}.
%
\subsection{Economical denial of sustainability} Online sandboxes, like any other business, have costs to sustain. Ignoring evasive malware to avoid an additional cost is (for now) understandable. Unfortunately, malware that exploits \name's technique implies additional energy and memory costs, especially if submitted in large scale to such systems, opening avenues to EDoS attacks, which will try to make the on-line service not sustainable economically. These on-line services receive on average 1.5M samples daily. It is not difficult to imagine how much energy just a tenth of the total submissions can consume if it is running PoW. Such algorithm is one of the most energy intensive operation that a computer can perform. For instance, the yearly energy consumption of Bitcoin's blockchain is comparable to the one of a country such as Tunisia or Czech Republic~\cite{bitpower}. We strongly recommend that not all evasion techniques are the same, and every technique that exploits hardware consumption side channels should be properly analyzed to avoid service disruption.

==> PoW for VM detection/08_related.tex <==
\section{Related Work}
\label{sec:related}
There is a significant body of research~\cite{c1,c2,c3,canali,DBLP:conf/ccs/LanziBKCK10,graziano,rotalume} focusing on both designing novel evasion techniques for malware and also providing mechanisms to detect them. We next discuss the most relevant works related to ours.
%
%\subsection{Evading Malware Analysis}
%Packer identification tools such as Yara and others~\cite{yara, rdg, peid} use  %%signatures to detect if an executable is packed with a specific previously known packer. %Moreover, these tools can be used in combination with manually written static unpackers %to enhance their functionality and customize their behaviour. Also, generic dynamic %unpackers have been proposed~\cite{omniunpack, renovo, codisasm} to avoid to write a %specific static unpacker which maybe useful for a single malware sample.
%Ugarte  \etal~\cite{ugarte} propose a taxonomy of packer complexity and perform a %exhaustive study of custom and COTS packers.
%In the work by D'Elia \etal~\cite{evamaldissect} a comprehensive description of %anti-analysis techniques, there is one of the first description on how to counter %stalling code which is one of the resilient anti-analysis technique and they claim the %approach to dismantle artifacts code is manual.
%
\point{Fingerprinting emulated environments}
%Several techniques have been proposed for fingerprinting the sandbox environment.
By recognizing the sandboxes of different vendors, malware can identify
the distinguishing characteristics of a given emulated environment and alter its behavior accordingly. 
The work in~\cite{1624022} introduced the notion of \emph{red  pill} and released a short exploit code snippet that could be used to detect whether the code is executed under a VM or in a real platform.  In~\cite{fistful}, the authors propose an automatic and systematic technique (based on EmuFuzzer~\cite{emufuzzer}) to generate red pills for detecting whether a program is executed inside a CPU emulator.
%Using this technique, the authors generated thousands of new red pills for two publicly available emulators, QEMU and BOCHS.
%
In~\cite{kemufuzzer}, the authors build KEmuFuzzer, which leverages protocol-specific fuzzing and differential analysis. KEmuFuzzer forces the hosting virtual machine and the underlying physical machine to execute specially crafted snippets of user- and system-mode code before comparing their behaviors. 
In~\cite{blackthorne} authors presented AVLeak, a tool that can fingerprint emulators running inside commercial antivirus (AV) software, which are used whenever AVs detect an unknown executable. The authors developed an approach that allows them to deal with these emulators as black boxes and then use side channels for extracting fingerprints from each AV engine.
Instead, we show that even with completely transparent analysis programs, the real environment can be used by the malware to determine that it is under analysis.
%
In~\cite{spotless_sand} authors propose a ML-based approach to detect emulated environments. This technique is based on the use of features such as the number of running processes, shared DLLs, size of temporary files, browser cookies, etc. These features are named by the authors ``wear-and-tear artifacts'' and are present in real system as opposed to sandboxes. The authors use such features to train an SVM classifier. We also rely on modeling a distinguishing feature, in our case is a time channel arising from the asymptotic behavior of a Pow, not the presence or absence of system artefacts.

%based on a PoW algorithm and takes a very small amount of time for detecting the emulated environment, without the need of performing an intensive training like in the case of SVM classifier. 

%Our idea is based on the available range of hardware platforms, we select a lower bound %(Raspberry Pi) and an upper bound (Intel I9). By using a statistical %technique~\cite{chebychev} on the distribution of the execution times of different %hardware platforms to compute the PoW algorithms; we are able to spot a sandbox within %only $10$ seconds with very high accuracy.

In~\cite{franklin2008remote}, authors introduce the virtual machine monitor (VMM) detection and they propose a fuzzy benchmark approach that works by making timing measurements of the execution time of particular code sequences executed on the remote system. The fuzziness comes from heuristics which they employ to learn characteristics of the remote system's hardware and its configuration. 
%In~\cite{DBLP:conf/isw/RaffetsederKK07}, authors analyze a number of %possibilities to detect system emulators. Their results show that emulation can %be successfully detected as easy as virtual machines, mainly because the task of %perfectly emulating real hardware is complex.
In~\cite{chen2008towards}, the authors present a technique that leverages TCP timestamps to detect anomalous clock skews in VMs. A downside of the approach is that it requires the transmission of streams of hundreds of SYN packets to the VM, something that can be detected in the case of a honeypot VM and flagged as malicious behavior. %Finally, in~\cite{ho2014tick} authors present a number of red pills based on timing side channels that are implemented in JavaScript and run in the browser, aiming to detect whether the browser is running inside a virtual machine. 
Compared to the previous approaches, \name is more principled and offers a solid basis founded on cryptographic primitives (PoW) with a predictable and reproducible computational behavior on different tested platforms.

\point{Detecting evasive malware}
In~\cite{dinaburg2008ether}, the authors propose Ether, a malware analyzer that eliminates in-guest software components vulnerable to detection. Ether leverages hardware virtualization extensions such as Intel VT, thus residing outside of the target OS environment. In \cite{barecloud}, the authors present an automated evasive malware detection system based on bare-metal dynamic malware analysis. Their approach is designed to be transparent and thus robust against sophisticated evasion techniques. The evaluation results showed that it could automatically detect 5,835 evasive malware out of 110,005 tested samples. In~\cite{balzarotti2010efficient}, authors propose a technique to detect malware that deploys evasion mechanisms. Their approach works by comparing the system call trace recorded when running a malware program on a reference system with the behavior observed in the analysis environment. In~\cite{lindorfer2011detecting}, authors propose a system for detecting environment-sensitive malware by comparing its behavior in multiple analysis sandboxes in an automated way. Compared to previous techniques, our approach is agnostic to system artifacts and cannot be recognized by only monitoring the system operations.

%\subsection{Timing Side Channels}
%%One of the most dangerous side channels is time, because algorithms have different %complexity and hence require more computational power and time to execute. The seminal %work on timing side-channels by Kocher~\cite{timingfoundational} dates back to 1996 and %the corpus of literature of these attacks is very huge, for the simple reason that %everything that has a clock consumes time. To the best of our knowledge the most recent %attack has been published by Huo \etal~\cite{bluethunder} against the Intel CPUs SGX %Trusted Execution Environment (TEE) which has been found to be vulnerable to %Foreshadow~\cite{foreshadow}. In general speculative execution features of CPUs expose %caches to timing side channels~\cite{meltdown, spectre}, in \name's case we don't exploit %micro architectural vulnerabilities, PoW is difficult enough to allow a more coarse %grained approach \ie for exploiting speculative execution a very high resolution timer is %required, in our case our resolution is in the order of $10^1$ seconds magnitude, which %makes the attack quite practical and easy to test.%

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\columnwidth]{figs/bitcoin_power.pdf}
%    \caption{Bitcoin PoW power consumption across time~\cite{bitpower}.}
%    \label{fig:bitpow}
%\end{figure}

%\subsection{Other Side Channels}
%Power consumption is also a way to spot something ``costly'' is happening in a machine, %the seminal work in this area appeared in 1999 by Kocher \etal~\cite{powerfoundational}. %PoW algorithms are well known to consume a lot of energy (as also shown in %Figure~\ref{fig:bitpow}), the Bitcoin network and its PoW yearly consumes roughly $70$ %%TeraWatts/hour on average, a figure comparable to a small country energy consumption \eg %Czech Republic~\cite{bitpower}. In the arms-race of malware also such side channel can be %exploited together with other features~\cite{spotless_sand} as a defence mechanism or %attack. Even though \name uses time to expose sandboxes because it does not require %very-high granular measurements. Also power consumption could be used to obtain a similar %result. As we show in Section~\ref{sec:defences} with respect to CPU usage%.


==> PoW for VM detection/09_conclusion_www.tex <==
\section{Conclusion}
\label{sec:conclusion}
Online malware scanning services are becoming more and more popular, allowing users to upload and scan artefacts against AV engines and malware analysis sandboxes.
Common mechanisms used by malware samples to avoid detection include the inspection of signals that imply the existence of a virtualized or emulated environment. These strategies triggered an arms-race where online malware scanners patch such signals to make virtualization transparent.
In this paper, we leverage PoW techniques as the basis for a novel malware evasion technique due to their ability to fingerprint real hardware. We provide empirical evidence of how it can be used to evade online malware analysis sandboxes and discuss potential countermeasures. The implementation of our approach goes beyond a simple proof-of-concept, showing that injecting evasion modules can be easily automated on any arbitrary sample. We make our code and results publicly available in an attempt to increase reproducibility and stimulate further research in this area.

==> PoW for VM detection/Preamble/macros.tex <==
\newcommand{\name}{\textsc{PoW-How}\xspace}
\newcommand{\etc}{{etc.}\xspace}
\newcommand{\etal}{{et al.}\xspace}
\newcommand{\eg}{{e.g.,}\xspace}
\newcommand{\ie}{{\it i.e.,}\xspace}
\newcommand{\rpi}{{Raspberry Pi 3}\xspace}
\newcommand{\point}[1]{\vspace{0.01in}\par\vspace{0.01in}\noindent{\textbf{#1:} }}
\newcommand\notes[1]{\textcolor{red}{#1}}
\newcommand{\authorsRef}{Antonio Nappa, Panagiotis Papadopoulos, Matteo~Varvello, Daniel Aceituno Gomez, Juan Tapiador, Andrea Lanzi\xspace}

% overwrite above decision if coming from Makefile
\ifdefined\nocomment
    \commentfalse
\fi

% RESULTS
\newcommand{\accuracy}{98.42\%\xspace}
\newcommand{\powTimeSec}{10 seconds\xspace}

%\newcommand{\note}[1]{\textcolor{red}{#1}}

\setlength\marginparwidth{16mm}
\setlength\marginparsep{1mm}
\setlength\marginparpush{2mm}

\makeatletter
\renewcommand\section{\@startsection
  {section}{1}{0mm}%name, level, indent
  {-\baselineskip} %             beforeskip
  {0.005\baselineskip}%            afterskip
{\bfseries}}% style
\makeatother

\makeatletter
\renewcommand\subsection{\@startsection
  {subsection}{2}{0mm}%name, level, indent
  {-0.3\baselineskip} %             beforeskip
  {0.005\baselineskip}%            afterskip
  {\bf\normalsize}}% style
\makeatother

\renewcommand\thesection{\arabic{section}.}
\renewcommand\thesubsection{\thesection\arabic{subsection}}

\def\UrlBreaks{\do\/\do-}
\sloppy
\raggedbottom

==> PoW for VM detection/Preamble/preamble.tex <==
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{enumitem}
\usepackage[style=base]{caption}
\usepackage{wrapfig}
\usepackage[T1]{fontenc}
\usepackage{mathtools}
\usepackage{subfigure}
\usepackage{enumitem,comment,wasysym}
\usepackage{color, soul}
\usepackage{pbox}
\usepackage{balance}
\usepackage{listings}
\usepackage{tikz,subfigure}
\usepackage{url}
\usepackage{booktabs} 
\usepackage{multirow}
\usepackage{xspace}
\usepackage{setspace}
\usepackage{hyperref}
\usepackage{hyphenat}
\usepackage{tablefootnote}
\usepackage{arydshln}
\usepackage{adjustbox}
\usepackage{tablefootnote}
\usepackage[stable]{footmisc}
\usepackage[most]{tcolorbox}
\usepackage{bibnames}
\usepackage[font=footnotesize,labelfont=bf]{caption}
%\usepackage[a4paper,twoside=false]{geometry}
\usepackage{times}

==> PoW for VM detection/old/background_long.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Background}
\label{sec:background}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Malware and Malware Analysis}
Malicious code has a large history in the field of Computer Science, its history goes along with the evolution of the technology that we use everyday. At the beginning computer networks were not existing and the way to infect machines was with vectors that were coming from media devices that would spread with the help of human interaction \ie borrow a floppy disk, a cd-rom or a usb key.~\cite{malwaremuseum}.
Once the Internet started to connect computers together the anatomy of malware changed drastically, they started to be called worms. These new software artifacts were capable of self reproducing and spreading around the network in an automated way~\cite{morrisworm}. The purpose of malicious interconnected software are several. Denial of service attacks, disrupting user experience, click-fraud and information exfiltration.


%In recent times we have seen the rise of Advanced Persistent Threats (APTs), which are targeted malware for specific organizations or governments to manipulate: politics, censorship and exfiltrate information~\cite{stuxnet}.
%Since the majority of economic transactions are moving towards the digital world, also the majority of capitals are being moved by on-line organizations. In particular, advertisement has become a fundamental pillar of the Internet economy. Advertisers get charged per impression per thousands of users or per click according to publisher's fares. Moreover if the click leads to a purchase the publisher can get an extra reward. It is fairly evident, that user privacy it is put at stake in such environment, though this goes beyond the scope of this paper. Here we are focusing on the evolution of malware, and in particular its relationship with the world of on-line advertisement has a strong connection with the botnet phenomenon. This network of infected computer is often sold as-a-service. Which means that someone can rent \eg 1M infected computers to perform fake clicks or generate a huge amount of traffic to disrupt a service.
%The advent of Bitcoin~\cite{bitcoin} and in general cryptocurrencies which allow anonymous payments has again mutated malware into a new species which is called Ransomware, a software which automatically spreads through the internet and encrypts all the data on the computer. To decrypt the data, malware authors ask for a ransom, that can be paid anonymously to several, untraceable, cryptocurrencies wallets.

%\begin{figure}[!th]
%\centering
%\includegraphics[width=0.6\columnwidth]{"figs/wannagraph.png"}
%\caption{WannaCry Ransomware variant dynamic execution graph (VirusTotal)}
%\label{fig:wannagraph}
%\end{figure}
%\point{Malware Analysis}
Together with the evolution of malicious software also researchers and professionals have reacted to improve their tools and skills to understand Malware and counter its consequences as fast as possible. There is a huge amount of literature devoted to analyze and counter malware~\cite{CyberProbe_NDSS14,autoprobe,Gu_ACSAC09_botProber,ppipup,ppi,Wang_Oakland10_TaintScope,DBLP:conf/sp/KolbitschHKK10,DBLP:conf/sp/MoserKK07}. Every aspect of the phenomenon has been taken into consideration, from its network infrastructure, to the code that gets reused among samples, unexplored paths in the control-flow, sandbox design and instrumentation. Nonetheless the arms race keeps running, while new analysis evasion techniques are found also new countermeasures get developed. 
%Figure~\ref{fig:wannagraph} gives an idea of how sandboxes environment can be useful to study malware samples and their behaviour. In this specific example we see that the WannaCry variant is contacting different servers between Europe and US to perform its operations.
%In general the figure gives an idea of the scale of the malware phenomenon and the amount of revenue that can be gained using infected machines.
\point{Anti-Analysis Techniques}
There are also several anti-analysis techniques which have been developed during the years by miscreants, and promptly countered by our community \eg packers~\cite{omniunpack,ugarte}, emulators~\cite{rotalume}, anti-debugging and anti-disassembly tricks and stalling code. Among all the techniques the only one that seems to resist is stalling code, this kind of technique is very difficult to detect and commercial sandboxes face the issue of this evasive measure~\cite{lastlinestall}.

\subsection{PoW as part of \name}
Proof-of-Work (PoW)~\cite{powdwork} is a consensus mechanism that requires some work from a client, which usually means computation time. A key feature of PoW algorithms is their asymmetry: the work imposed on the client is moderately hard but it is easy for a server to check the computed result. There are two types of PoW protocols: (a) \emph{challenge-response} protocols, which require an % direct 
interactive link between the server and the client, and (b) \emph{solution-verification} protocols, which allow the client to solve a self-imposed problem and send the solution to the server to verify the validity of the problem and its solution. Such %problems 
PoW protocols (also known as CPU cost functions) leverage algorithms like hashcash with double iterated SHA256~\cite{laurie2004proof}, momentum birthday collision~\cite{larimer2014momentum}, cuckoo cycle~\cite{tromp2015cuckoo}, and more. These algorithms may be:

\begin{enumerate}
    \item  {\bf Memory-bound}, where computation speed is bound by main memory accesses. The performance of such algorithms is expected to be less sensitive to hardware evolution.

    \item {\bf CPU-bound}, where computation speed is bound by the system's processor, which greatly varies in time, as well as between high-end and low-end devices.

    \item {\bf Network-bound}, where a client must collect tokens from remote nodes before querying the service provider. In this sense, the work is not performed by the client, but they incur delays because of the latency to get the required tokens.
\end{enumerate}

%PoW has gained much popularity in recent years by becoming the founding block of the blockchain technology. PoW is the (trustless) consensus algorithm in a blockchain network that is used to confirm transactions and append new blocks to the chain. In particular, performing PoW---which in this context is known as mining---is required as a way to force miners to compete against each other in solving complex computational puzzles. Whenever a miner solves the PoW computational puzzle of a new block, (s)he broadcasts that block to the network. All other miners can then easily verify that the solution is correct and the block will be confirmed. The difficulty of each PoW puzzle is periodically adjusted to keep the block construction time around a target time~\cite{powdwork}.
%\jetnote{[minor] a reference here would be welcome.}

%\subsection{Catena, Argon2, and Yescrypt}
While designing \name, we considered three PoW implementations: (1) Catena~\cite{catena}, (2) Argon2~\cite{argon2,argon2rfc} and (3) Yescrypt~\cite{yescrypt}. These algorithms were among the finalists of the Password Hashing Competition (PHC)~\cite{phc,wetzels2016open,phc2}, which led to the design of significant improvements in the PoW implementation, namely stability in memory footprint, duration, and CPU usage. 

\subsubsection{The choice of Argon2} 
 Argon2 won PHC and it is the PoW strategy used in \name. Argon2 guarantees that, by using the same input parameters, the amount of computation performed is asymptotically constant; hence, the variance of Argons2's execution time $T$ is very small on the same platform. Moreover, Argon2 is based on a memory-hard function which, even in the case of parallel or specialized execution (\eg ASICs or FPGAs), will not enhance scalability, and hence 
 remains computationally bounded due to its asymptotic behavior. The Argon2 algorithm takes the following inputs:
 \begin{itemize}
     \item A message string $P$, which is a password for password hashing applications. Its length must be within 32-bit size.
     \item A nonce $S$, which is used as salt for password hashing applications. Its length must be within 32-bit size. 
     \item A degree of parallelism $p$ that determines how many independent (but synchronized) threads can be run. Its value should be within 24-bit size (minimum is 1).
     \item A tag, which length should be within 2 and 32-bit %length.\jetnote{what's this for?}
     \item A memory size $m$, which is a number expressed in Kibibytes
    %\footnote{A “Kibibyte” is equal to 1024, or $2^{10}$, bytes. It is a %new term to discern between the Kilo prefix in the universal metric %system which normally represents a $10^3 (1000)$ magnitude factor. %While in Computer Science that corresponds to $2^{10}$ which is 1024 %so the name Kilobyte should be 1000 bytes and has always been %interpreted as 1024 in reality.\jetnote{I don't think this %explanation is needed.}} $8*p$ to within 32bit. The actual number of %blocks is $m^\prime$, which is $m$ rounded down to the nearest %multiple of $4*p$.
     \item A number of internal iterations $t$, which is used to tune the running time independently of the memory size. Its value should be within 32-bit size (minimum is 1).
 \end{itemize}

%*****************************************************WOOT CUT***************************************************************
 These input parameters will be used in our framework to define the computational boundary of the algorithm execution on a specific class of hardware machine. Once the parameters are set, the output of the PoW algorithm only depend on the hardware platform. 
% %\jetnote{Since we don't describe how the algorithm works, motivate why describing the inputs %is interesting.} 
 Argon2 has two implementations: Argon2d and  Argon2i. Argon2d maximizes resistance to GPU-based password cracking attacks~\cite{bakker2010gpu} by accessing the memory array in a data-dependent order, which reduces the possibility of time–memory trade-off (TMTO) attacks~\cite{1056220}. 
 Argon2d accesses the memory array in a data-dependent order to maximize its resistance against GPU-based password cracking attacks~\cite{bakker2010gpu}. Another benefit of this access pattern is that it also reduces the possibility of time–memory trade-off (TMTO) attacks~\cite{1056220}. However, this comes with the associated cost of being vulnerable to side-channel attacks~\cite{wetzels2016open}. Conversely, Argon2i does not have data-dependency (\ie the next iteration of the algorithm does not depend on the previous one) and thus it is resilient against such attacks. As a consequence, Argon2i became popular as a PoW in cryptocurrencies and back-end servers as it makes it difficult to observe memory patterns. Argon2i is our choice for \name evasion for its security features (\eg memory protection against side channel).


%*****************************************************WOOT CUT***************************************************************




%\jetnote{Why is Argon2 described in greater detail than Catena and %Yescrypt if the three are supported in the tool?}
Here are the main features of the algorithm:
\begin{enumerate}
    \item \textbf{Performance}: the selected memory area is filled very fast, this plays against adversaries with specialized ASIC.
    \item \textbf{Tradeoff Resilience}: with default number of memory passes an ASIC equipped adversary can not decrease the time-area product even if the memory size used is reduced by a factor of 4 of more. This has been proved not to work with Catena and Lyra algorithms.
    \item \textbf{GPU-FPGA-ASIC Unfriendly}: implementing a dedicated cracking hardware will not improve performances (timewise) of the algorithm.
\end{enumerate}

%Argon2 uses its own compression function G which takes two 1024-byte inputs and a 1024-byte output. Also, it uses its own hash function $H^x()$ with x being its output length in bytes. $H^x()$ applied to the input string A is the BLAKE2b~\cite{blake} function. %\begin{figure}[t]

%\begin{figure}[b!]
%    \centering
%    \includegraphics[scale=.4]{figs/argon_op.pdf}
%    \caption{Argon2 (single thread) mode of operation.}
%    \label{fig:argon2op}
%end{figure}

%, which takes (d,|dd|,kk=0,nn=x) as parameters. Where d is the initial input string A padded to a multiple of 128 bytes and partitioned into 128-byte blocks. Function G is based on the permutation of the blocks derived from BLAKE2b output. 


%The reason, is that Argon2d uses as new input of its next iteration the previous output of the algorithm, hence a malicious observer could introspect or use a side-channel to accelerate artificially the calculus. 

%Figure~\ref{fig:argon2op} explains in a nutshell the internals of the algorithm. The compression function $G$ starts with two 1024 bytes blocks $block(i)$ and $block(i+1)$, and will output a single 1024 bytes output block $(i+1)$. Function $G$ is based on permutations of the Blake2b~\cite{blake} hash function. $G$ is iterated $x$ times and at each step $i$ the next block is either derived from previous output if Argon2d (data-dependent) is used, or taken from memory if Argon2i is used.
Our choice of Argon2 is motivated by the results shown in Section~\ref{sec:eval}. 

 \point{Catena and Yescrypt}
 In \name we also consider the other two PoW algorithms: Catena and Yescrypt, since our goal is to show that such class of algorithms shared the same computational behavior and can be used for fingerprinting the hardware platform. We refer the reader to their respective publications~\cite{catena,yescrypt} for further information.

\subsection{Timing side channels vs. Stalling Code vs. \name's Approach}
Various technique have been proposed to detect if applications are running inside a sandbox/virtualizer/emulator, among them the most reliable are based on timing measurements~\cite{timingfoundational}. Indeed fine grained timers help also to build micro-architectural attacks such as Spectre and Meltdown~\cite{meltdown,spectre}. Also, stalling code (e.g. long or infinite loops) maybe helpful to thwart instrumented execution which normally have execution timeouts.
The intuition behind our work is that PoW algorithms offer strong cryptographic premises with a very stable complexity growth, which make the approach very resilient to any countermeasure, such as using more powerful bare-metal machines to enhance performance and reduce the space for time measurements.

By exploiting the asymptotic behavior of the PoW algorithms, we build a statistical model that can be used to guess the class of environment where the algorithm is running and consequently distinguish between physical and virtualized, emulated or simulated architectures, like different flavors of malware sandboxes.
Indeed, even fine grained red-pills techniques~\cite{fistful} such as CPU instruction misbehaviour can be easily fixed in the sandbox or spoofed to thwart evasion techniques. On the other hand PoW stands on top of well defined mathematical and well defined computational behaviour. Moreover, a simple modification of the PoW library avoids the malware sample to be fingerprinted with statical techniques. If we take as an example of PoW complexity, the one that is run in the crypto currency environment, we know that by design the computation complexity of the algorithm is increased for each new block of the blockchains transaction~\cite{bitcoin}. For instance, the PoW used by blockchain, its computation complexity increases for each new block of blockchains transactions~\cite{bitcoin}. %This is due to the fact that resources (cryptocoins) of the blockchain ecosystem are limited; as the resources availability decreases, their price in terms of computational power grows, hence the PoW computation becomes more difficult at every iterations.
Such increasing of computation show the asymptotic behavior that can be exploited by our technique. %To approve a pool of transactions an amount of computation is needed to solve the PoW and compute the next block of the chain. 
By applying PoW as a malware sandbox evasion technique we get an off-the-shelf technique which, improves the resilience malware and limits its analysis. %Figure~\ref{fig:bitpow} shows Bitcoin's PoW minimal power consumption (dashed line) and expected power consumption (solid line) in TeraWatt/year. The figure transmits two important challenges faced by the PoW algorithms when applied in the blockchain context. First, the number of Bitcoin transactions increase every day and hence checking their validity quickly is crucial (\eg the algorithm should use the entire hardware resources for responding quickly). Second, over time it is possible to see that the power consumption increases; this is due to the implementation of the algorithm which becomes more and more difficult since it needs to consider more data at time and require an extra computational power, for every new transaction pool till reach the computational saturation. To understand how expensive are such algorithms, a news article~\cite{bbc} claims that Bitcoin's power consumption is already in world's top 30 overcoming countries such as Argentina, Netherlands and UAE. 
%Section~\ref{sec:defences} shows how timers can be spoofed to try to thwart \name's approach.
%\begin{figure}[h!]
%\centering
%\includegraphics[width=\columnwidth]{"figs/bitcoin_power"}
%\caption{Bitcoin Proof-of-Work - TeraWatt/Year}
%\label{fig:bitpow}
%\end{figure}
%\paragraph{Proof-of-Work Algorithm.}
%%In general PoW is a consensus mechanism, a fault-tolerant policy %that allows a distributed system to keep its correct state even in %presence of faulty nodes~\cite{powdwork}. The principle behind any %PoW algorithm in a distributed system is that there is a challenge %response mechanism and the challenger asks its counterpart to solve a %computationally moderate-hard challenge to compute that requires an %amount of work (computation). %Another important characteristic of %PoW algorithms is the high %speed at which the challenger can prove %the work has been made %\ie checking a simple hash. 
%%This is normally important for blockchains because of the magnitude %of transaction that are normally made. 
%\mvnote{I feel like this was already said before?}\anote{integrated %in the above paragraph}


==> PoW for VM detection/old/introduction_old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In 2016, the global cost of malware-based attacks had reached a staggering \$450 billion dollars~\cite{malwarecost2016}. It took only 2 years for the economic toll of cyber-crime to reach 
\$1.5 trillion dollars (or \$2.9 million dollars per minute)~\cite{malwarecost2018}, with predictions 
hinting at this cost to reach \$6 trillion dollars by 2021~\cite{malwareCost}. 

Due to the sheer amount of known malware samples~\cite{virushare, virustotalstats},  manual analysis neither scales nor allows to build any comprehensive threat intelligence around the detected cases (\eg malware clustering by specific behavior, family or infection campaign). To address this problem, security researchers have introduced \emph{sandboxes}~\cite{anubis}: isolated environments that automate the dynamic execution of malware and monitor its behavior under different scenarios. Sandboxes usually comprise a set of virtual machines instrumented to gather fundamental information of the malware execution such as: system calls, registry keys accessed/modified, new files created, memory patterns. Such techniques are extensively used by antivirus companies or online scanning services (\eg VirusTotal) that analyze malware samples submitted by users. More recently, sandboxes have also become critical for checking mobile app submissions to online app marketplaces~\cite{sandboxandroid}. 
%Apart from the sandbox that monitors the behavior of the malware, in %some cases, the malware itself is monitoring its environment to detect %the presence of a sandbox. So called \emph{evasive} malwares use various %sophisticated techniques to detect virtualized environments and pause %the delivery of their malicious payload. %thus evading detection. 

As malware analysis systems become more widely used, miscreants constantly search for new methods to evade detection. To achieve this, they alter the execution behavior of their code and pause the delivery of any malicious payload when it runs on an emulated environment. A first step towards this direction for the malware is to recognize accurately whether it resides on a sandbox environment or a real user device.  The \emph{red-pill}~\cite{1624022} is a popular technique to detect virtualized environments by leveraging CPU instructions that are not properly emulated. The success of this approach motivated later works~\cite{fistful,kemufuzzer} to automate the process of generating red-pills. Similar techniques propose the exploitation of specific devices or registry keys, memory patterns or parallel running processes of known VM vendors (\eg VMWare, VirtualBox)~\cite{vmware, vbox}. A more general and advanced technique is proposed in~\cite{spotless_sand}, where the authors design an empirical ML-based technique to detect emulated environments. The approach is based on several system features (DLLs, browser cookies, \etc) that are used for training an SVM classifier and detect sanboxing environments. 

These evasion techniques triggered an arms-race with malware analysts to design countermeasures which eliminate or spoof the ``signals'' that red pill techniques exploit~\cite{barecloud}. On the other hand, attackers use (trusted) crowd-sourced malware scanning services (like VirusTotal or similar online services~\cite{sandboxes}) as a testbed to measure and tune the evasiveness of their malware. Indeed, there are  cases~\cite{graziano} where malware authors abused such services for testing their evasion mechanisms before distributing their malicious software to people.\alnote{I think here, we need to say why we need another evasion technique or better position our technique respect to the others that already exists, something like we are more agnostic, we do not depend on the specific characteristic of the software implementation of the sandbox etc.}

In this paper we introduce a novel malware evasion technique 
to create an exploitable {\it timing side-channel attack} that is able to recognize whether the malware is running on an emulated environment. To this end we design an automatic tool called  \name\footnote{A disguising suite described in the book ``A Scanner Darkly'' by Philip K. Dick~\cite{darkly}} that is a three-steps pipeline framework which executes multiple Proof-of-Work~\cite{powdwork} (POW) algorithms (e.g., blockchain technology) on several hardware platforms, and applies a statistic inequality to properly estimate the amount of time
necessary to execute such algorithms on real hardware.   In the first step of the pipeline, our framework estimates a PoW threshold that is a statistical characterization of the execution time of different PoW algorithms that run on different hardware platform. This step allows the system to select some algorithm parameters (second step) that will be used along with the PoW execution for detecting the sandbox environment and finally in the last step the system will embed in the malware the PoW algorithm with the selected parameters and run a testbed on sandbox environment to evaluate the accuracy of the sandbox detection. PoW algorithms are very suitable for such a model since, once the input parameters are fixed, their execution time only depends on a machine’s available CPU and memory (e.g, side-channel timing attack).
\jetnote{The previous par needs an additional pass to better describe the technique.}
%In this paper, we present \name\footnote{A disguising suite described in the book %``A Scanner Darkly'' from Philip K. Dick~\cite{darkly}}: a novel VM-detection %approach 
%that is effective even when the malware cannot identify neither instrumentation nor %introspection artifacts 
%at run time. \name leverages \emph{stalling code}~\cite{kruegbh,lastlinestall} to %create exploitable {\it timing side-channels attack} that is able to recognize %whether the malware is running on emulated environment (\eg sandbox). 

%This is achieved via off-the-shelf Proof-of-Work (PoW)~\cite{powdwork} algorithms (\eg blockchain technology) which stress the host and trigger hardware discrepancies. In particular {\it \name runs PoW algorithms and builds up a statistical model that is able to discern on which classes of hardware-machine (\eg real or simulated) the algorithm is running on}. 
%MV -- attempted at merging the two above sentences since this paragraph is quite long and the concept was, imho, quite similar 

%This is achieved combining off-the-shelf Proof-of-Work %(PoW)~\cite{powdwork} algorithms (\eg blockchain technology) with a %statistical model that is able to discern on which classes of %hardware-machine (\eg real or simulated) the algorithm is running %on. PoW algorithms are very suitable for such a model since, once %the input parameters are fixed, their execution time only depends on %a machine's available CPU and memory. %specific hardware machine %resources: CPU and memory usage. 
A key advantage of the evasion technique deployed by \name is that it relies on benign PoW implementations and thus it does not raise suspicion to automated malware sandboxes. Moreover, current techniques aimed at spoofing the virtualization signals present in contemporary sandboxes cannot act as countermeasures against the timing side-channels that \name exploits.

To asses the feasibility and effectiveness of \name,
%three-steps pipeline framework,
we wrote a malware PoC that implements some standard ransomware activities (e.g., scanning and encryption of files). The sample also embeds a PoW algorithm with a configuration chosen by \name. To select the appropriate PoW parameters, we ran our framework on three different hardware platforms: a low-end (Raspberry Pi 3), a medium-end (Dual Intel Xeon), and a high-end (Intel i9) machine with two different OSes (Linux Ubuntu 18.1 and Windows 10). We assumed two operational settings CPU-wise, idle and busy, to estimate a threshold that could distinguish a real hardware platform from a sandbox emulated environment. The results show that our malware sample is able to successfully evade the real sandboxes that recognize it as a benign sample.
\jetnote{Missed: which sandboxes was this tested against?}

%To asses the feasibility and effectiveness of \name, we compare %three different PoW algorithms and we implement a proof of %concept of our approach using Argon2 PoW %implementation~\cite{argon2, poc}. We integrate our prototype %into a real %malware sample (\eg 
%ransomware which delivers its malicious payload only if the %probability of running in a sandbox is low enough. We evaluate %the effectiveness of our approach on several physical and %virtual machines (Intel Core i9, Raspberry Pi, VirtualBox, %JoeSandbox and VirusTotal). Our evaluation results demonstrate %that in the best case our technique can guess the sandbox %environment in \powTimeSec with \accuracy accuracy.

\noindent{\bf Contributions.} The contributions of this paper can be summarized in the following: 

\begin{enumerate}
    \item We design \name, an automatic three-steps pipeline framework which executes multiple PoW algorithms on several hardware platforms, and applies a statistical model to properly distinguish between the real hardware platform and the emulated ones. To increase the awareness of the community we release the source code of our system \footnote{https://github.com/Raid2020Submission/Submission63}.
    
    %\item We compare the performance of 3 different Proof-of-Work algorithms on different hardware platforms and operating systems.
    
    %\item We implement a proof of concept of our approach that %utilizes the Argon2 algorithm which we integrate %our proof of concept 
    %into a real ransomware.% sample. 

    \item We evaluate the effectiveness of \name by running our prototype on executing the PoW configuration on three different hardware platforms: Raspberry Pi 3, Dual Intel Xeon, and Intel i9 machines with two different OSes Linux Ubuntu 18.1 and Windows 10 and assuming two state conditions:  idle and busy (CPU-wise). Results show the effectiveness of our method.
    
    %Our results show that \name can detect a sandbox with  \accuracy of %accuracy with an execution time of \powTimeSec.
    
    \item We perform a security analysis of our tool and we discuss limitations and potential countermeasures of our systems that could improve the defensive approach against such evasion technique. Moreover, we show how our technique can be applied in new fingerprint contexts.
\end{enumerate}


==> PoW for VM detection/old/old-04_approach.tex <==
\begin{figure*}[th]
\centering
    \includegraphics[scale=.65]{"figs/System-Design.pdf"}
    \caption{Experiment Design - 1. Ansible playbook start - 2. Execution of three PoW algorithms (Argon2, Catena, YesCrypt) on different HW platforms - 3. Bounding of threshold for PoW execution to evade sandboxes - 4. Compilation and Test }
\label{fig:arch}
\end{figure*}
%MV -- compress the figure by removing all that whitespace. 

%\section{Implementation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Evading Sandboxes with \name}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This section describes \name design and implementation.
\name is a pipeline which executes at least three different PoW algorithms, on several hardware platforms, and applies the Chebyshev~\cite{chebychev} inequality to estimate properly the amount of time necessary to execute the PoW on real hardware. \mvnote{Before reaching here, the reader is kinda confused of what \name is. Is it an evasion mechanism, is it a testbed, is it an evasive malware? We need to somehow unify the writing.} \anote{it is not a malware, is it an automated tool to evade malware sandboxes, and it works end to end from threshold calculation to malware production, we changed title also because of that reason, I rephrased a bit also}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{PoW Threshold Estimation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We start by describing the tool we built to statistically estimate PoW thresholds, \ie quantify the execution times of different PoW runs on real hardware. We have chosen three of the finalists algorithms of the password hashing competition PHC~\cite{phc} for our case. In particular we have selected, Argon2 (the winner), Catena and Yescrypt. %The choice of the last two is mostly due to their good coding practices %which eased the integration in \name.

A single run of this tool involves the execution of the three different PoW algorithms  multiple times with different input parameters. %, has already explained in Section~\ref{sec:background}.
The repetition of the executions is necessary to obtain statistical meaning and significance. In a nutshell, the parameters of the algorithm allow to select the amount of memory, parallelism and complexity of the PoW. Our selection was based on common configuration of COTS hardware devices, with respect to cores, memory and CPU. However, not all the selected algorithms have these parameters available for tuning and in some cases their tuning is more coarse grained~\cite{catena}.
Next, we benchmarked \name over three hardware platforms representative of high-end, medium-end, and low-end platforms. Our high-end hardware is a desktop equipped with an Intel(R) Core(TM) i9-9900X CPU @ 3.50GHz with 10 physical cores and 20 threads equipped with an PCI-e M2 512GB disk, 32 GB of fast access RAM.
Our medium-end is a workstation equipped with a Dual Intel(R) Xeon(R) CPU E5-2643 0 @ 3.30GHz with 16 physical cores and 64GB of RAM. Finally our low-end device is a RaspberryPi3 which comes equipped with a quad core ARMv7 Processor rev 4 (v7l) and 1GB of RAM.
The idea is to produce an equal number of samples per hardware platform (300) and apply the Bienaymé–Chebyshev inequality~\cite{chebychev}%  this inequality allows to establish how much of the sample population of unknown statistical distribution is contained within a distance from the mean $\mu$.
%To be more accurate the results of the Bienaymé–Chebyshev inequality 
, which shows the percentage of the population contained between K times $\sigma$ from the mean $\mu$.

The formula $Pr(|X - \mu| \geq k\sigma) \leq \frac{1}{k^2}$ allows to select a threshold $T$ (e.g., execution time) which for \name's experimental evaluation can encompass up to 99.1\% of the sample population, see Table~\ref{tab:catena}. For our evaluation we have selected Argon2i~\cite{argon2, argon2rfc} which guarantees a 98.3\% sample population coverage.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Malware Integration.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Once \name completes the tests, it automatically calculates the threshold to evade detection based on the hardware platforms used to build its model. Our Malware PoC is written in VC++ for Windows 10 and in C++ for Linux and is roughly~150 LoC. It implements a simple ransomware which scans the entire hard drive and encrypts all its files. The idea is that the malicious behaviour is exposed only if the Argon2 PoW will be executed at least T times before a timer expires. We leverage also the Boost libraries~\cite{boost} to ease the OS interaction and build a single statically-linked executable. We selected Argon2 because from our experiments it emerges that in only ten seconds it is possible to evince whether the platform on which the executable is running is real hardware or an instrumented VM. The complete compilation step is automated as an Ansible~\cite{ansible} playbook and clang~\cite{clang}, this pipeline installs the Ansible scripts runs the tests and starts to compile the malware binary for multiple platforms automatically.

==> PoW for VM detection/old/old-06_evaluation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Evaluation}
\label{sec:eval}
%%%%%%%%%%%%%%%%%%%%%%%%%
In this section, we leverage \name to evaluate the effectiveness of associating a PoW with  evasive malware. We start by empirically quantifying the execution time of popular PoWs on a spectrum of devices. Next, we built an actual ransomware which leverages the execution time of Argon2i (the PoW we have chosen, see Section~\ref{sec:background}) as an evasion mechanism, and show its effectiveness when tested on JoeSandbox~\cite{joesandbox},  Hybrid-Analysis~\cite{hanalysis}, and VirusTotal~\cite{virustotal}. 
%we have tested extensively three PoW algorithms and established solid statistical bounds to evade behavioural malware sandbox in a methodical and repeatable way.

For each PoW currently supported by \name, we have selected different configurations with respect to memory footprint, parallelism and algorithm internal iterations. All the details are in Tables~\ref{tab:argon},~\ref{tab:catena},~\ref{tab:yescrypt}. Argon2i and Yescrypt have similar parameters, like memory, number of threads, blocks, while Catena's only parameter is a graph size which grows in memory and will make its computation harder %with respect to the graph size.
as the graph size increases. 

We execute each PoW configuration on the low-end, medium-end, and high-end machines available to \name. For starters, we execute each PoW configuration for about 24 hours on each machine under optimal conditions on Linux Ubuntu 18.04.3, \ie no additional load present on the machines. 
%If additional load on the machine were considered, PoW algorithm could %perform less than usual and consequently this would just lower the %upper bound. In any case the lower bound of the Windows machine that %runs PoW algorithm in not  optimal conditions is still different in %execution time as showed in Table~\ref{tab:malhw2}. %Such lower bound is quite hard to accomplish since the difference in %terms of PoW cycles between the sandbox with the other machines is %quite hi. In this case the malware could test the PoW estimation in %different random time windows to avoid the load and detect the correct %hardware machine computation power. 
%Though, results show that to perform worse or equal than a sandbox you probably %need to use one of them and overload it. %according to an estimation performed %in optimal conditions. 
Table~\ref{tab:hw_totals} shows that, over 24 hours, both the high and medium-end platforms completed 9,000 executions of each PoW configuration (9 in total) on each platform. In comparison, the low-end platform (RaspBerry Pi 3) only completed 300 executions. The same algorithms perform worse on the same machine on Windows 10 in dual boot configuration. To validate our results on this worst case we perform an experiment where we run our malware that embeds PoW algorithm on Windows 10 machine in not optimal condition (\eg CPU-Z), see the results in Table~\ref{tab:malhw2}. Even in this worst case the Windows machine performs better than any sandboxes in terms of power execution time, Table~\ref{tab:malsand}.


%Hence, to establish a good upper bound we have selected the best %platform \ie Linux in terms of results.

%These results establish our basis to extrapolate statistical bounds on how much time $T$ is needed to detect a sandbox environment, with respect to the number of PoW that can be executed during $T$.


%In Tables~\ref{tab:argon},\ref{tab:catena},\ref{tab:yescrypt} we show the results of an unknown statistical distribution of 900 samples for the three platform. The results of the Bienaymé–Chebyshev inequality shows the percentage of the population contained between K times $\sigma$ from the mean $\mu$, according to Bienaymé–Chebyshev~\cite{chebychev} inequality $Pr(|X - \mu| \geq k\sigma) \leq \frac{1}{k^2}$.

Next, we aim at statistically investigate each PoW execution times distribution  obtained across our platforms. To do so, we leverage the Bienaymé–Chebyshev inequality. To balance equally sized data-sets, we sampled 300 random executions (\ie the total number of executions that were possible on the low-end platform) from the 9,000 executions available from both the medium and high-end platforms.  %results of the other two platforms 300 random results to obtain a uniform sample size for the three platforms.
Tables~\ref{tab:argon},~\ref{tab:catena},~\ref{tab:yescrypt} show for each PoW and configuration, several statistics (min, max, $\sigma$, and $K$, Chebyshev inequality) computed over an unknown statistical distribution of 900 execution times obtained across the three platform. The results of Chebyshev inequality show the effectiveness of the idea behind \name. With different execution parameters we were able to detect each platform with high accuracy (98\%, on average), independently of whether we are consider low-end, medium-end, or high-end hardware. %the real hardware machine architecture population represent by low-end medium-end and high-end platform.   

%Since within a small time frame it is possible to discern on which %hardware platform the PoW was executed. 
%~\mvnote{the last sentence does not read well, but was not sure how to %fix.}\anote{fixed, take a look}

Table~\ref{tab:malhw1}, summarizes the results of running \name's automated malware implementation on both Microsoft Windows 10 and Linux Ubuntu 18.04.3. We consider both the 32 and 64 bit configurations, and optimal conditions. We have included the Argon2i PoW in our PoC ransomware~\cite{ransomware}. The idea is, since for Argon2i the minimum execution time of one run of the algorithm (see Table~\ref{tab:argon} second line) on the Intel i9 is 0.2 seconds and the maximum is 9.28 under optimal conditions. \anote{@matteo check last sentence} The malware should be able to execute 50 execution of the PoW in 10 seconds. As we can evince from Table~\ref{tab:malhw1} the results are way below the expectancy on Windows 10 64bits, operated in optimal conditions. The malware PoC is able to perform only on average 28.3 executions of the proof during 10 seconds. The Linux operating system remains a point of reference because its execution times are better and hence it provides a better upper bound for \name's implementation. ~\mvnote{is this related to the impact of non being under optimal conditions? Instead of present like this, should we first remove that assumption, show this result, and then move to the next step?}\anote{this is related to the operating system, both were in idle state, it's just that windows does worse, I reorganized a bit the text}

The above results suggest us to set the evasive condition to trigger after $T=10$ seconds and check if at least $x$ number of the PoW have been completed. We have submitted different variants of the sample to different sandboxes and the results are disheartening, none of the sandbox is able to execute more than 1 cycle of the PoW, leaving a huge space of improvements of such environments.
Table~\ref{tab:malsand}, shows the results of our malware executions on sandboxes, which are normally Windows based. Which give complete results of behavioural analysis. Our malware PoC is not packed, and hence, some of the behaviour is visible through exported functions. Even though none of the samples was flagged as malicious.
The most interesting lines of Table~\ref{tab:malsand}, are the ones were we test the sandbox to perform better than a native Intel i9 and extend their time of execution to the available maximum (if possible) and double the timeout \eg $T=20 x=15$.
None of the tested sandboxes was able to perform any better of a simple RaspBerry pi. Which is a very modest hardware machine. All the reports of our analysis are publicly available, including screenshots of evasive malware samples~\cite{eva1, eva2, eva3, eva4, eva5, evavt, evavtsgamo}. While the report of same sample analyzed without evasive measure is available here~\cite{noteva, mal_vt}. It has to be noted that VirusTotal's sandbox report is not very detailed as JoeSandbox, but they both show the hard drive scan (Ransomware behaviour). Also, in Table~\ref{tab:malsand} the number of PoW executed is visible only if a screenshot of the sandbox is available. Also, with respect to the sandbox execution timeout. Both available only on JoeSandbox.
\begin{center}
\begin{table}
\caption{Full execution of 3 PoW Macro-Behchmark Results (Linux Ubuntu) }
\label{tab:hw_totals}
\centering
\begin{tabular}{|r|r|l|}
\hline
 \# Runs &  Total (hours) &  Platform\\
\hline
9,000 & 22.33 & Intel i9-9900X 3.50GHz \\
\hline
9,000 & 29.47 & Dual Intel Xeon E5-2643 3.30GHz \\
\hline
300 & 24.59 & RaspBerry Pi 3 \\
\hline
\end{tabular}
\end{table}

\begin{table*}
             \caption{Results for Argon2i Algorithm (Linux Ubuntu)}
             \label{tab:argon}
             \centering
\begin{tabular}{|r|l|r|r|r|r|r|r|c|}
\hline
 Threads & Internal Iterations & Memory & Min &  Max &  Sigma &  Mean &    K &  Chebyshev\\
\hline
 1 & 10 & 1024 KiB & 0.01 & 0.70 &  0.09 &  0.02 & 7.89 & 98.39\% \\
 \hline
 8 & 100 & 4096 KiB & 0.20 & 9.28 &  1.09 & 0.48 & 8.09 & 98.34\% \\ 
 \hline
 16 & 500 & 8192 KiB &  2.03 & 88.80 &  10.68 &  3.91 & 7.95 & 98.42\% \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\caption{Results for Catena Algorithm (Linux Ubuntu)}
\label{tab:catena}
\centering
\begin{tabular}{|c|r|r|r|r|c|c|}
\hline
 Garlic Graph Size & Min &  Max &  Sigma &  Mean &  K & Chebyshev \\
\hline
15 & 0.12 & 5.35 &   0.51 &  0.21 & 9.99 &          99.00\% \\
\hline
18 & 1.13 & 35.61 &   4.25 &  1.88 & 7.94 &          98.41\% \\
\hline
20 & 5.11 & 165.57 &  19.03 &  8.28 & 8.26 &          98.54\% \\
\hline
\end{tabular}
\end{table*}

\begin{table*}
\caption{Results for Yescrypt Algorithm (Linux Ubuntu)}
\label{tab:yescrypt}
\centering
\begin{tabular}{|r|r|r|r|r|r|r|c|c|}
\hline
 Threads & Blocks & Block Size & Min &  Max &  Sigma &  Mean &    K &  Chebyshev \\
\hline
1 & 1024 & 8KB & 0.00 & 0.02 &   0.00 &  0.01 & 6.14 &  97.35\% \\
\hline
8 & 2048 & 32KB & 0.03 & 0.56 &   0.05 &  0.05 & 10.52 & 99.10\% \\
\hline
16 & 4096 & 64KB & 0.08 & 5.00 &   0.51 &  0.19 & 9.39 & 98.87\% \\
\hline
\end{tabular}
\end{table*}
\end{center}


\begin{table*}
\caption{Malware Execution Results on Hardware (Idle) }
\label{tab:malhw1}
\centering
\begin{tabular}{|r|r|c|c|c|c|c}
\hline
Machine & Timeout & $\mu$ of \# PoW Win32 & $\mu$ of \# PoW Win64 & $\mu$ of \# PoW Linux32 & $\mu$ of \# PoW Linux64 \\
\hline
Intel i9 & 10sec & 17.5 & 28.3 & 33.2 & 48.2\\
\hline
Intel i7 & 10sec & 11.2  & 17.2 & 23.3 & 38.1\\ 
\hline
Dual Xeon & 10sec & 10.1  & 15.3 & 20.2 & 44.2\\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\caption{Malware Execution Results on Hardware (Busy with CPU-Z on Windows)}
\label{tab:malhw2}
\centering
\begin{tabular}{|r|r|c|c|c|c|c}
\hline
Machine & Timeout & $\mu$ of \# PoW Win32 & $\mu$ of \# PoW Win64\\
\hline
Intel i9 & 10sec & 15.5 & 23.5\\
\hline
Intel i7 & 10sec & 9.2  & 15.1\\ 
\hline
Dual Xeon & 10sec & 12.2 & 13.4 \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\caption{Malware Execution Results on Sandboxes}
\label{tab:malsand}
\centering
\begin{tabular}{|r|r|c|c|c|c|}
\hline
Sandbox & Evasion Timeout & PoW Check condition &\# of PoW executed & Execution Timeout & Notes\\
\hline
JoeSandbox & $10 secs$ & 50 & 1 & 120 & Clean\\
\hline
JoeSandbox & $15 secs$ & 45 & 1 & 180 & Clean\\
\hline
JoeSandbox & $20 secs$ & 40 & 1 & 240 & Clean\\
\hline
JoeSandbox & $20 secs$ & 15 & 1 & 500 & Clean\\
\hline
Hybrid-Analysis & $20 secs$ & 15 & 0 & Not available & Clean\\
\hline
VirusTotal & $20 secs$ & 45 & Not available & Not available & Clean\\
\hline
VirusTotal & $20 secs$ & 15 & Not available & Not available & Clean\\
\hline
\end{tabular}
\end{table*}


==> PoW for VM detection/old/old-11_discussion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Security Analysis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The previous section demonstrates that a \name(ed) malware successfully evades popular sandbox environments. This is achieved by associating a PoW (Argon2d) with the malware, whose downside is an increase in both CPU and memory consumption. Figure~\ref{fig:cpueva} and~\ref{fig:mem_footprint}  compare, respectively,  CPU and memory utilization of our malware (red line) with \texttt{connhost.exe} (Console Windows Host) as reported by XXX. With respect to the CPU usage, the PoW associated with our malware causes an (expected) 100\% utilization for the whole duration of the PoW ($T$). With respect to  memory utilization, our malware only require about 17~MB versus, for instance, 7~MB that utilizes a sample system process like \texttt{connhost.exe}.


\begin{figure}[t]
\centering
    \tcbox[top=0pt,left=0pt,right=0pt,bottom=0pt]{{\includegraphics[scale=.45]{"figs/cpu_evader.png"}}}
    \caption{CPU Consumption of Malware PoC (Argon2d) Malware:red line connhost.exe:green line }
\label{fig:cpueva}
\end{figure}


\begin{figure}[t]
\centering
    \tcbox[top=0pt,left=0pt,right=0pt,bottom=0pt]{{\includegraphics[scale=.45]{"figs/evader_mem.png"}}}
    \caption{Memory Consumption of Malware PoC (Argon2d) Malware:red line connhost.exe:green line}
\label{fig:mem_footprint}
\end{figure}

To further investigate the impact of the above increase in CPU and memory usage of   gather 


We have tested also benign programs which are, surprisingly flagged as suspicious, while our malware is flagged as clean. In Figure~\ref{fig:cpu_z} we show the execution of the CPU-Z utility~\cite{cpuz} to fingerprint and test CPUs. This is clearly flagged as a suspicious program especially because of its CPU consumption and the multiple submission the sample has had~\cite{cpuz_eva}.

\begin{figure}[th]
\centering
    \tcbox[top=0pt,left=0pt,right=0pt,bottom=0pt]{{\includegraphics[scale=.321]{"figs/cpu_z.png"}}}
    \caption{CPU Consumption of CPU-Z Utility, CPU-Z:red line connhost.exe:green line}
\label{fig:cpu_z}
\end{figure}

We have further tested countermeasures to reduce the CPU usage of our PoC ransomware. First we have reduced the PoW execution and the timeout $T$ to 3 seconds and obtained less CPU drain, with a peak of 80\% as it is possible to see in Figure~\ref{fig:evader_ant}. The complete report is available here~\cite{mal_ant1}. This reduces the suspiciousness of the sample but, using such a small $T = 3$ seconds, reduces also the margin to evade the sandbox and hence easily detectable.

\begin{figure}[th]
\centering
    \tcbox[top=0pt,left=0pt,right=0pt,bottom=0pt]{{\includegraphics[scale=.321]{"figs/evader_ant.png"}}}
    \caption{CPU Consumption of Malware PoC $T=3$ seconds, Malware:red line connhost.exe:green line}
\label{fig:evader_ant}
\end{figure}

As another approach we have tried is make our PoW to go low-and-slow, by setting $T = 60$ seconds and a sleep of $.5$ seconds between each execution of the PoW. Figure~\ref{fig:evader_ant2} yet, shows a very high CPU usage, which means that to obtain a smoother curve the sleep has to last more time. However this would transform our PoW approach into an effective stalling code solution, which sleeps. The report is available here~\cite{mal_ant2}. Moreover since the plots are coming directly from the sandbox the sleeping time could be not sufficient with respect to their measurement sampling rate of CPU drain.


\begin{figure}[th]
\centering
    \tcbox[top=0pt,left=0pt,right=0pt,bottom=0pt]{{\includegraphics[scale=.321]{"figs/evader_ant2.png"}}}
    \caption{CPU Consumption of Malware PoC $T=60$ seconds, Malware:red line connhost.exe:green line}
\label{fig:evader_ant2}
\end{figure}

We also compare the behavioural maps of our malware PoC vs CPU-Z in Figures~\ref{fig:subpoc} and ~\ref{fig:subcpuz} and as it is possible to see, CPU-Z is clearly shown as a false positive from the sandbox. Indeed, CPU-Z is a more complex software respect to a simple ransomware that scans the hard drive and encrypts every file. Though, it does not have anything malicious in it.

\begin{figure}[ht]
\centering
\begin{subfigure}
  \centering
  \includegraphics[scale=.3]{figs/evader.png}
  \caption{Malware PoC Behavioural Map}
  \label{fig:subpoc}
\end{subfigure}

\begin{figure}
    \centering
    \includegraphics[scale=.3]{figs/naked.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}



%
\begin{subfigure}
  \centering
  \includegraphics[scale=.3]{figs/benign.png}
  \caption{CPU-Z Behavioural Map}
  \label{fig:subcpuz}
\end{subfigure}
\end{figure}

Another important aspect to underline, of Figures~\ref{fig:subpoc} and~\ref{fig:subcpuz} is that our Malware PoC is neither packed nor stripped, and hence some of its functionality \ie exported functions, linked libraries, and function names are visible through basic static analysis as noted before. With some extra effort our zero-day malware would be undetectable for a good amount of time and its behavioural map would look even greener. Raising the detection bar even more.

==> PoW for VM detection/old/old_00_abstract.tex <==
\begin{abstract}
Malware analysis systems are one of the best weapons in the arsenal of cybersecurity companies and researchers. An integral part of such systems is a sandbox providing an instrumented and isolated environment to run unknown artefacts and observe their behavior to identify potentially malicious actions. In order to avoid detection, attackers have developed numerous techniques to make analysis harder. One class of anti-analysis attacks is based on the observation that it is not only the sandbox that monitors the behavior of the running program; the program itself can also monitor its surrounding environment to detect the presence of a sandbox and try to evade it. This is usually achieved by looking for artifacts suggesting that the execution environment is a sandbox, such as specific memory patterns, behavioral traits of certain CPU instructions (known as red pills), or parallel running processes of known Virtual Machine (VM) vendors. To mitigate this threat, sophisticated sandboxes remove or spoof these signals, thus making it harder for a malware sample to detect the emulated environment.
In this paper we devise a new evasion strategy based on Proof-of-Work (PoW) algorithms that show an asymptotic behavior, in terms of computational cost, when they run on some class of hardware platform. To this end such algorithms can be used to effectively detect virtualized environment (e.g., malware sandbox analysis). To prove the validity of this intuition, we design and implement \name: a tool that is able to automatically implement such detection strategies and embed a test evasion program into an arbitrary malware sample. Evaluation results show that the proposed detection technique can evade the most popular public sandboxes.
\end{abstract}

%The reason of using PoW implementations is that they put under heavy load physical machines and have, according to our results, higher accuracy in distinguishing machines used by legit users with respect to sandboxes, depending on their execution time. 

==> PoW for VM detection/old/old_01_introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\$1.5 trillion dollars (or \$2.9 million dollars per minute)~\cite{malwarecost2018}, with predictions 
hinting at this cost to reach \$6 trillion dollars by 2021~\cite{malwareCost}. 

Due to the sheer amount of known malware samples~\cite{virushare, virustotalstats},  manual analysis neither scales nor allows to build any comprehensive threat intelligence around the detected cases (\eg malware clustering by specific behavior, family or infection campaign). To address this problem, security researchers have introduced \emph{sandboxes}~\cite{anubis}: isolated environments that automate the dynamic execution of malware and monitor its behavior under different scenarios. Sandboxes usually comprise a set of virtual machines instrumented to gather fundamental information of the malware execution, such as system calls, registry keys accessed/modified, new files created, and memory patterns. Such techniques are extensively used by antivirus companies or online scanning services (\eg VirusTotal) that analyze malware samples submitted by users. Sandboxes have also become critical for mobile app for online marketplaces~\cite{sandboxandroid}. 
%Apart from the sandbox that monitors the behavior of the malware, in %some cases, the malware itself is monitoring its environment to detect %the presence of a sandbox. So called \emph{evasie} malwares use various %sophisticated techniques to detect virtualized environments and pause %the delivery of their malicious payload. %thus evading detection. 

Sandboxing is only successful at detecting malicious behavior if it goes undetected. If a malware sample can detect the presence of a sandbox, it can simply abort the execution of any malicious payload. The \emph{red pill}~\cite{1624022,fistful,kemufuzzer} is a popular technique to detect virtualized environments by leveraging CPU instructions, registry keys, memory patterns, and other artifacts that are not correctly emulated. Regardless of the specific technique used, the above detection mechanism does not work in advanced sandboxes that can spoof the ``signals'' that red pill techniques exploit~\cite{barecloud}. This has motivated miscreants to use (trusted) crowd-sourced malware scanning services (like VirusTotal or similar online services~\cite{sandboxes}) as a testbed to measure and adjust the evasiveness of their malware programs. 
More recently, \cite{spotless_sand} proposes to use several system features (DLLs, browser cookies, \etc) to train an SVM classifier and detect sandboxing environments. Such a technique needs a training phase based on a real environment and it should exactly know which system resources need to be considered.

In this work, we introduce a new set of evasion strategies based on Proof-of-Work (PoW)~\cite{powdwork} algorithms. Our intuition lies on the fact that, like NP-class problems~\cite{npp}, the asymptotic behavior of a PoW algorithm is constant in terms of computational cost~\cite{powdwork}, \eg CPU and memory consumption. Accordingly, PoW algorithms are perfect candidates for benchmarking the capability of the hardware where they are run, revealing the absence or presence of a sandbox because of the deviation with respect to the expected measured performance.
%Moreover, current techniques aimed at spoofing the virtualization signals present in contemporary sandboxes cannot act as countermeasures against the timing side-channels that \name exploits.
A key advantage of using PoW techniques is that they are self-contained mechanisms compared to the other more fine-grained timing side-channel approaches. In fact, it does not require the access to precise timing resources for detecting the emulated environment (e.g., network or fine-grained timers). The technique is robust enough since it can detect the
emulated environment with high precision just by looking at the output of the algorithm, as we will show in the experiments.
Moreover, it relies on PoW implementations that do not raise any suspicion to automated malware sandboxes. While stalling code e.g. (infinite loops and/or sleep) are easier to detect because of CPU idleness. Fingerprinting PoW algorithm as a malware component is feasible e.g. by checking the usage of particular cryptographic instructions. Though, it can produce a huge number of false positive compared with more fine-grained ad-hoc side-channel techniques~\cite{10.1145/2818000.2818030}. This because PoW algorithms can be part of a legit application.
Using the above idea, we built \name,\footnote{A disguising suite described in the book ``A Scanner Darkly'' by Philip K. Dick~\cite{darkly}} a framework to automatically create, inject, and evaluate PoW-based evasion strategies in arbitrary programs. \name operates as a three-steps pipeline. During the fist step, multiple PoW algorithms are tested across different hardware platforms (Raspberry Pi 3, Dual Intel Xeon, Intel i9), operating systems (Linux Ubuntu 18.03 and Windows 10), and machine loads. These extensive tests are used to build a statistical characterization of each PoW execution time in each setting, using the Bienaym\'{e}–Chebyshev inequality~\cite{chebychev} to obtain sound statistics about the expected execution time. In the next step, a miscreant can upload its malware to \name and select the evasion mechanism to be used. Finally, \name automatically evaluates the accuracy of the evasion mechanism selected, when coupled with the uploaded malware, via several tests run both on a local sandbox and on multiple on-line free-of-charge sandbox services~\cite{sandboxes}.

We empirically evaluate each step of \name's pipeline. For the PoW threshold estimation, we have tested three popular PoW algorithms
(Catena~\cite{catena}, Argon2~\cite{argon2,argon2rfc} and Yescrypt~\cite{yescrypt}) using multiple configurations. During 24 hours of testing, we find Chebyshev inequality values higher than 97\% regardless of the PoW and configuration. This confirms high determinism in the PoW execution times on real hardware, thus validating the main intuition behind this work.
We test our technique over two known ransomware families by submitting to VirusTotal several variants that include PoW-based evasion. The results demonstrate how the inclusion of this mechanism reduces the number of detections, even in the presence of other anti-analysis techniques such as code virtualization or packing.
To further analyze its impact on real-world analysis sandboxes, we wrote a  fully functional malware sample, integrated an evasion mechanism based on Argon2, and submitted it to JoeSandbox~\cite{joesandbox}, Hybrid-Analysis~\cite{hanalysis}, and VirusTotal~\cite{virustotal}). Reports from each sandbox all mark our malware as \emph{clean}, validating the effectiveness of a PoW-based evasion mechanisms. We further discuss the behavioral analysis reported by JoeSandbox for our malware, as well as potential countermeasures to this novel PoW-based evasion mechanism we have proposed.

In order to increase the reproducibility of our results and foster further research on this topic, we make the source code of our system publicly available.\footnote{\url{https://github.com/anonnymousubmission/anonymousubmission}}

%\footnote{https://github.com/Raid2020Submission/Submission121}

\paragraph{Organization.}
The rest of this paper is organized as follows. Section~\ref{sec:background} provides some background on PoW algorithms. Section~\ref{sec:framework} introduces our evasion framework, which is evaluated in Section~\ref{sec:eval} against real-world malware sandboxing services. Section~\ref{sec:analysis} discusses in detail the behavioral reports obtained from the sandboxes, and Section~\ref{sec:defences} discusses possible countermeasures. Sections~\ref{sec:related} and \ref{sec:ethics} discuss related work and ethical considerations, respectively. Finally Section~\ref{sec:conclusion} concludes the paper summarizing our main contributions and discussing future work.

==> PoW for VM detection/old/old_09_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
\name represents one further step in the evolution of evasion techniques for malware. We believe that the application of PoW as a malware evasion technique is an innovative and provocative idea, exposing a weaknesses in our current analysis platforms. In this paper, we have provided empirical evidence of how it can be used to evade real-world malware analysis sandboxes, and discussed potential countermeasures. Furthermore, our implementation of \name goes beyond a simple PoC, showing that injecting evasion modules can be easily automated on any arbitrary sample. We make our code and results publicly available in an attempt to increase reproducibilty and stimulate further research in this area.
%Malicious software has become very complex, and often very targeted. all the techniques that are used to evade, thwart and ultimately avoid detection are often inherited from different samples or derived from particular vulnerabilities of the specific target. However, \name shows a new generic technique that can be used maliciously to avoid detection and indirectly foster the expansion of malicious software to new unprotected victims. For this reason is very important to act and find viable countermeasures against such principled approaches which could really change the way malware is executed and exposes its behaviour. We have proposed several techniques that can help to mitigate such attack.


%Indeed, PoW is the ultimate frontier to avoid attacks to distributed systems such as %blockchain and its power has been demonstrated through the fact that transactions %cannot be replayed and crypto-coins cannot be double spent. 
%Moreover, \name goes beyond a simple PoC, showing that it can be easily automated %and expose weaknesses and limitations of malware analysis platforms, in a principled, methodical and repeatable way. 
%Moreover \name shows that is able to fingerprint a sandbox within only $10$ seconds in a %way that cannot be fixed with a simple workaround. 
%Indeed, combining \name with a good packing technology, which could be an %emulator~\cite{rotalume} or a known twist of existing packers~\cite{ugarte} can make %dynamic analysis quite hard. 

%On the other hand, as we mention as countermeasure techniques there are possibilities to %fingerprint PoW algorithms inside malware. Also enhancing sandboxes to execute crypto %operations, on which PoW are based, natively even if the virtualized environment is %instrumented can help to raise the bar. 
%In Section~\ref{sec:futures} we evaluate potential enhancements of \name and defences %against it.


%\point{Future Work}
%\label{sec:futures}
%\paragraph{Malware Automation}
%Our aim is to continue to study the phenomena that surrounds malware, its analysis, and the countermeasures that can be applied to thwart such analysis. We envision that attack-driven research is a necessary approach to demonstrate the duality of every phenomena that are in conflict. In this specific case we think that malware could in the future, thwart analysis directly trying to mine the last block of a public blockchain as some JS based malware was doing to get rewarded. In this case, the mining would serve as stalling code to evade detection. Moreover, updates to the malware evasion time can be done on the fly when the next block of the blockchain is calculated, thus automating the evasive behavior upgrade.

%\paragraph{CPU Fingerprinting}
%With a very granular source of time, given the asymptotic behavior of the PoW algorithms we believe that they may be used to fingerprint hardware platforms instead of simply distinguishing sandboxes from real hardware. The potential of this proposal is to perform such fingerprinting remotely as Sánchez-Rola~\cite{clock} did, \ie through the browser. This opens many new questions about user profiling, privacy and security. However, since the well-known micro-architectural bugs Spectre, Meltdown, and Foreshadow~\cite{spectre, meltdown, foreshadow} the timer resolution granularity of browsers, normally accessed through the $performance.now()$ JavaScript function~\cite{perfNow} has been highly reduced, so fingerprinting a specific CPU based on execution time can become a daunting task and requires a lot of time or generate many false positives.

==> PoW for VM detection/old/unused_05_implementation.tex <==
\section{Implementation}
Implementation is divided in two phases, first we will describe the implementation of the testbed and its execution program. Second we will describe an implementation of a potential ransomware program which leverages PoW as an evasion measure. All the code of the implementation is available at~\cite{poc}.
\paragraph{Testbed Implementation.}
The test program has been implemented in Python3 language with approximately 100 LoC. Every experiment has been designed to last approximately a single day based on the hardware capabilities of the machines. For each PoW we have tested three different configuration which we will accurately describe in the Section~\ref{sec:evaluation}. In a nutshell the different parameters allow to select the amount of memory, parallelism and complexity of the PoW. We repeated the experiment as much as possible during approximately 24 hours to obtain meaningful statistics.
\paragraph{Malware Implementation.}
Our PoC is written in VC++ for Windows 10 and is roughly ~150 LoC. It implements an example of a ransomware, which scans the entire hard drive and encrypts all the files into it. The idea is that the malicious behaviour is exposed only if the Argon2 PoW will be executed at least T times before a timer expires. 
\label{sec:implementation}

==> old/background_long.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Background}
\label{sec:background}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Malware and Malware Analysis}
Malicious code has a large history in the field of Computer Science, its history goes along with the evolution of the technology that we use everyday. At the beginning computer networks were not existing and the way to infect machines was with vectors that were coming from media devices that would spread with the help of human interaction \ie borrow a floppy disk, a cd-rom or a usb key.~\cite{malwaremuseum}.
Once the Internet started to connect computers together the anatomy of malware changed drastically, they started to be called worms. These new software artifacts were capable of self reproducing and spreading around the network in an automated way~\cite{morrisworm}. The purpose of malicious interconnected software are several. Denial of service attacks, disrupting user experience, click-fraud and information exfiltration.


%In recent times we have seen the rise of Advanced Persistent Threats (APTs), which are targeted malware for specific organizations or governments to manipulate: politics, censorship and exfiltrate information~\cite{stuxnet}.
%Since the majority of economic transactions are moving towards the digital world, also the majority of capitals are being moved by on-line organizations. In particular, advertisement has become a fundamental pillar of the Internet economy. Advertisers get charged per impression per thousands of users or per click according to publisher's fares. Moreover if the click leads to a purchase the publisher can get an extra reward. It is fairly evident, that user privacy it is put at stake in such environment, though this goes beyond the scope of this paper. Here we are focusing on the evolution of malware, and in particular its relationship with the world of on-line advertisement has a strong connection with the botnet phenomenon. This network of infected computer is often sold as-a-service. Which means that someone can rent \eg 1M infected computers to perform fake clicks or generate a huge amount of traffic to disrupt a service.
%The advent of Bitcoin~\cite{bitcoin} and in general cryptocurrencies which allow anonymous payments has again mutated malware into a new species which is called Ransomware, a software which automatically spreads through the internet and encrypts all the data on the computer. To decrypt the data, malware authors ask for a ransom, that can be paid anonymously to several, untraceable, cryptocurrencies wallets.

%\begin{figure}[!th]
%\centering
%\includegraphics[width=0.6\columnwidth]{"figs/wannagraph.png"}
%\caption{WannaCry Ransomware variant dynamic execution graph (VirusTotal)}
%\label{fig:wannagraph}
%\end{figure}
%\point{Malware Analysis}
Together with the evolution of malicious software also researchers and professionals have reacted to improve their tools and skills to understand Malware and counter its consequences as fast as possible. There is a huge amount of literature devoted to analyze and counter malware~\cite{CyberProbe_NDSS14,autoprobe,Gu_ACSAC09_botProber,ppipup,ppi,Wang_Oakland10_TaintScope,DBLP:conf/sp/KolbitschHKK10,DBLP:conf/sp/MoserKK07}. Every aspect of the phenomenon has been taken into consideration, from its network infrastructure, to the code that gets reused among samples, unexplored paths in the control-flow, sandbox design and instrumentation. Nonetheless the arms race keeps running, while new analysis evasion techniques are found also new countermeasures get developed. 
%Figure~\ref{fig:wannagraph} gives an idea of how sandboxes environment can be useful to study malware samples and their behaviour. In this specific example we see that the WannaCry variant is contacting different servers between Europe and US to perform its operations.
%In general the figure gives an idea of the scale of the malware phenomenon and the amount of revenue that can be gained using infected machines.
\point{Anti-Analysis Techniques}
There are also several anti-analysis techniques which have been developed during the years by miscreants, and promptly countered by our community \eg packers~\cite{omniunpack,ugarte}, emulators~\cite{rotalume}, anti-debugging and anti-disassembly tricks and stalling code. Among all the techniques the only one that seems to resist is stalling code, this kind of technique is very difficult to detect and commercial sandboxes face the issue of this evasive measure~\cite{lastlinestall}.

\subsection{PoW as part of \name}
Proof-of-Work (PoW)~\cite{powdwork} is a consensus mechanism that requires some work from a client, which usually means computation time. A key feature of PoW algorithms is their asymmetry: the work imposed on the client is moderately hard but it is easy for a server to check the computed result. There are two types of PoW protocols: (a) \emph{challenge-response} protocols, which require an % direct 
interactive link between the server and the client, and (b) \emph{solution-verification} protocols, which allow the client to solve a self-imposed problem and send the solution to the server to verify the validity of the problem and its solution. Such %problems 
PoW protocols (also known as CPU cost functions) leverage algorithms like hashcash with double iterated SHA256~\cite{laurie2004proof}, momentum birthday collision~\cite{larimer2014momentum}, cuckoo cycle~\cite{tromp2015cuckoo}, and more. These algorithms may be:

\begin{enumerate}
    \item  {\bf Memory-bound}, where computation speed is bound by main memory accesses. The performance of such algorithms is expected to be less sensitive to hardware evolution.

    \item {\bf CPU-bound}, where computation speed is bound by the system's processor, which greatly varies in time, as well as between high-end and low-end devices.

    \item {\bf Network-bound}, where a client must collect tokens from remote nodes before querying the service provider. In this sense, the work is not performed by the client, but they incur delays because of the latency to get the required tokens.
\end{enumerate}

%PoW has gained much popularity in recent years by becoming the founding block of the blockchain technology. PoW is the (trustless) consensus algorithm in a blockchain network that is used to confirm transactions and append new blocks to the chain. In particular, performing PoW---which in this context is known as mining---is required as a way to force miners to compete against each other in solving complex computational puzzles. Whenever a miner solves the PoW computational puzzle of a new block, (s)he broadcasts that block to the network. All other miners can then easily verify that the solution is correct and the block will be confirmed. The difficulty of each PoW puzzle is periodically adjusted to keep the block construction time around a target time~\cite{powdwork}.
%\jetnote{[minor] a reference here would be welcome.}

%\subsection{Catena, Argon2, and Yescrypt}
While designing \name, we considered three PoW implementations: (1) Catena~\cite{catena}, (2) Argon2~\cite{argon2,argon2rfc} and (3) Yescrypt~\cite{yescrypt}. These algorithms were among the finalists of the Password Hashing Competition (PHC)~\cite{phc,wetzels2016open,phc2}, which led to the design of significant improvements in the PoW implementation, namely stability in memory footprint, duration, and CPU usage. 

\subsubsection{The choice of Argon2} 
 Argon2 won PHC and it is the PoW strategy used in \name. Argon2 guarantees that, by using the same input parameters, the amount of computation performed is asymptotically constant; hence, the variance of Argons2's execution time $T$ is very small on the same platform. Moreover, Argon2 is based on a memory-hard function which, even in the case of parallel or specialized execution (\eg ASICs or FPGAs), will not enhance scalability, and hence 
 remains computationally bounded due to its asymptotic behavior. The Argon2 algorithm takes the following inputs:
 \begin{itemize}
     \item A message string $P$, which is a password for password hashing applications. Its length must be within 32-bit size.
     \item A nonce $S$, which is used as salt for password hashing applications. Its length must be within 32-bit size. 
     \item A degree of parallelism $p$ that determines how many independent (but synchronized) threads can be run. Its value should be within 24-bit size (minimum is 1).
     \item A tag, which length should be within 2 and 32-bit %length.\jetnote{what's this for?}
     \item A memory size $m$, which is a number expressed in Kibibytes
    %\footnote{A “Kibibyte” is equal to 1024, or $2^{10}$, bytes. It is a %new term to discern between the Kilo prefix in the universal metric %system which normally represents a $10^3 (1000)$ magnitude factor. %While in Computer Science that corresponds to $2^{10}$ which is 1024 %so the name Kilobyte should be 1000 bytes and has always been %interpreted as 1024 in reality.\jetnote{I don't think this %explanation is needed.}} $8*p$ to within 32bit. The actual number of %blocks is $m^\prime$, which is $m$ rounded down to the nearest %multiple of $4*p$.
     \item A number of internal iterations $t$, which is used to tune the running time independently of the memory size. Its value should be within 32-bit size (minimum is 1).
 \end{itemize}

%*****************************************************WOOT CUT***************************************************************
 These input parameters will be used in our framework to define the computational boundary of the algorithm execution on a specific class of hardware machine. Once the parameters are set, the output of the PoW algorithm only depend on the hardware platform. 
% %\jetnote{Since we don't describe how the algorithm works, motivate why describing the inputs %is interesting.} 
 Argon2 has two implementations: Argon2d and  Argon2i. Argon2d maximizes resistance to GPU-based password cracking attacks~\cite{bakker2010gpu} by accessing the memory array in a data-dependent order, which reduces the possibility of time–memory trade-off (TMTO) attacks~\cite{1056220}. 
 Argon2d accesses the memory array in a data-dependent order to maximize its resistance against GPU-based password cracking attacks~\cite{bakker2010gpu}. Another benefit of this access pattern is that it also reduces the possibility of time–memory trade-off (TMTO) attacks~\cite{1056220}. However, this comes with the associated cost of being vulnerable to side-channel attacks~\cite{wetzels2016open}. Conversely, Argon2i does not have data-dependency (\ie the next iteration of the algorithm does not depend on the previous one) and thus it is resilient against such attacks. As a consequence, Argon2i became popular as a PoW in cryptocurrencies and back-end servers as it makes it difficult to observe memory patterns. Argon2i is our choice for \name evasion for its security features (\eg memory protection against side channel).


%*****************************************************WOOT CUT***************************************************************




%\jetnote{Why is Argon2 described in greater detail than Catena and %Yescrypt if the three are supported in the tool?}
Here are the main features of the algorithm:
\begin{enumerate}
    \item \textbf{Performance}: the selected memory area is filled very fast, this plays against adversaries with specialized ASIC.
    \item \textbf{Tradeoff Resilience}: with default number of memory passes an ASIC equipped adversary can not decrease the time-area product even if the memory size used is reduced by a factor of 4 of more. This has been proved not to work with Catena and Lyra algorithms.
    \item \textbf{GPU-FPGA-ASIC Unfriendly}: implementing a dedicated cracking hardware will not improve performances (timewise) of the algorithm.
\end{enumerate}

%Argon2 uses its own compression function G which takes two 1024-byte inputs and a 1024-byte output. Also, it uses its own hash function $H^x()$ with x being its output length in bytes. $H^x()$ applied to the input string A is the BLAKE2b~\cite{blake} function. %\begin{figure}[t]

%\begin{figure}[b!]
%    \centering
%    \includegraphics[scale=.4]{figs/argon_op.pdf}
%    \caption{Argon2 (single thread) mode of operation.}
%    \label{fig:argon2op}
%end{figure}

%, which takes (d,|dd|,kk=0,nn=x) as parameters. Where d is the initial input string A padded to a multiple of 128 bytes and partitioned into 128-byte blocks. Function G is based on the permutation of the blocks derived from BLAKE2b output. 


%The reason, is that Argon2d uses as new input of its next iteration the previous output of the algorithm, hence a malicious observer could introspect or use a side-channel to accelerate artificially the calculus. 

%Figure~\ref{fig:argon2op} explains in a nutshell the internals of the algorithm. The compression function $G$ starts with two 1024 bytes blocks $block(i)$ and $block(i+1)$, and will output a single 1024 bytes output block $(i+1)$. Function $G$ is based on permutations of the Blake2b~\cite{blake} hash function. $G$ is iterated $x$ times and at each step $i$ the next block is either derived from previous output if Argon2d (data-dependent) is used, or taken from memory if Argon2i is used.
Our choice of Argon2 is motivated by the results shown in Section~\ref{sec:eval}. 

 \point{Catena and Yescrypt}
 In \name we also consider the other two PoW algorithms: Catena and Yescrypt, since our goal is to show that such class of algorithms shared the same computational behavior and can be used for fingerprinting the hardware platform. We refer the reader to their respective publications~\cite{catena,yescrypt} for further information.

\subsection{Timing side channels vs. Stalling Code vs. \name's Approach}
Various technique have been proposed to detect if applications are running inside a sandbox/virtualizer/emulator, among them the most reliable are based on timing measurements~\cite{timingfoundational}. Indeed fine grained timers help also to build micro-architectural attacks such as Spectre and Meltdown~\cite{meltdown,spectre}. Also, stalling code (e.g. long or infinite loops) maybe helpful to thwart instrumented execution which normally have execution timeouts.
The intuition behind our work is that PoW algorithms offer strong cryptographic premises with a very stable complexity growth, which make the approach very resilient to any countermeasure, such as using more powerful bare-metal machines to enhance performance and reduce the space for time measurements.

By exploiting the asymptotic behavior of the PoW algorithms, we build a statistical model that can be used to guess the class of environment where the algorithm is running and consequently distinguish between physical and virtualized, emulated or simulated architectures, like different flavors of malware sandboxes.
Indeed, even fine grained red-pills techniques~\cite{fistful} such as CPU instruction misbehaviour can be easily fixed in the sandbox or spoofed to thwart evasion techniques. On the other hand PoW stands on top of well defined mathematical and well defined computational behaviour. Moreover, a simple modification of the PoW library avoids the malware sample to be fingerprinted with statical techniques. If we take as an example of PoW complexity, the one that is run in the crypto currency environment, we know that by design the computation complexity of the algorithm is increased for each new block of the blockchains transaction~\cite{bitcoin}. For instance, the PoW used by blockchain, its computation complexity increases for each new block of blockchains transactions~\cite{bitcoin}. %This is due to the fact that resources (cryptocoins) of the blockchain ecosystem are limited; as the resources availability decreases, their price in terms of computational power grows, hence the PoW computation becomes more difficult at every iterations.
Such increasing of computation show the asymptotic behavior that can be exploited by our technique. %To approve a pool of transactions an amount of computation is needed to solve the PoW and compute the next block of the chain. 
By applying PoW as a malware sandbox evasion technique we get an off-the-shelf technique which, improves the resilience malware and limits its analysis. %Figure~\ref{fig:bitpow} shows Bitcoin's PoW minimal power consumption (dashed line) and expected power consumption (solid line) in TeraWatt/year. The figure transmits two important challenges faced by the PoW algorithms when applied in the blockchain context. First, the number of Bitcoin transactions increase every day and hence checking their validity quickly is crucial (\eg the algorithm should use the entire hardware resources for responding quickly). Second, over time it is possible to see that the power consumption increases; this is due to the implementation of the algorithm which becomes more and more difficult since it needs to consider more data at time and require an extra computational power, for every new transaction pool till reach the computational saturation. To understand how expensive are such algorithms, a news article~\cite{bbc} claims that Bitcoin's power consumption is already in world's top 30 overcoming countries such as Argentina, Netherlands and UAE. 
%Section~\ref{sec:defences} shows how timers can be spoofed to try to thwart \name's approach.
%\begin{figure}[h!]
%\centering
%\includegraphics[width=\columnwidth]{"figs/bitcoin_power"}
%\caption{Bitcoin Proof-of-Work - TeraWatt/Year}
%\label{fig:bitpow}
%\end{figure}
%\paragraph{Proof-of-Work Algorithm.}
%%In general PoW is a consensus mechanism, a fault-tolerant policy %that allows a distributed system to keep its correct state even in %presence of faulty nodes~\cite{powdwork}. The principle behind any %PoW algorithm in a distributed system is that there is a challenge %response mechanism and the challenger asks its counterpart to solve a %computationally moderate-hard challenge to compute that requires an %amount of work (computation). %Another important characteristic of %PoW algorithms is the high %speed at which the challenger can prove %the work has been made %\ie checking a simple hash. 
%%This is normally important for blockchains because of the magnitude %of transaction that are normally made. 
%\mvnote{I feel like this was already said before?}\anote{integrated %in the above paragraph}


==> old/introduction_old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In 2016, the global cost of malware-based attacks had reached a staggering \$450 billion dollars~\cite{malwarecost2016}. It took only 2 years for the economic toll of cyber-crime to reach 
\$1.5 trillion dollars (or \$2.9 million dollars per minute)~\cite{malwarecost2018}, with predictions 
hinting at this cost to reach \$6 trillion dollars by 2021~\cite{malwareCost}. 

Due to the sheer amount of known malware samples~\cite{virushare, virustotalstats},  manual analysis neither scales nor allows to build any comprehensive threat intelligence around the detected cases (\eg malware clustering by specific behavior, family or infection campaign). To address this problem, security researchers have introduced \emph{sandboxes}~\cite{anubis}: isolated environments that automate the dynamic execution of malware and monitor its behavior under different scenarios. Sandboxes usually comprise a set of virtual machines instrumented to gather fundamental information of the malware execution such as: system calls, registry keys accessed/modified, new files created, memory patterns. Such techniques are extensively used by antivirus companies or online scanning services (\eg VirusTotal) that analyze malware samples submitted by users. More recently, sandboxes have also become critical for checking mobile app submissions to online app marketplaces~\cite{sandboxandroid}. 
%Apart from the sandbox that monitors the behavior of the malware, in %some cases, the malware itself is monitoring its environment to detect %the presence of a sandbox. So called \emph{evasive} malwares use various %sophisticated techniques to detect virtualized environments and pause %the delivery of their malicious payload. %thus evading detection. 

As malware analysis systems become more widely used, miscreants constantly search for new methods to evade detection. To achieve this, they alter the execution behavior of their code and pause the delivery of any malicious payload when it runs on an emulated environment. A first step towards this direction for the malware is to recognize accurately whether it resides on a sandbox environment or a real user device.  The \emph{red-pill}~\cite{1624022} is a popular technique to detect virtualized environments by leveraging CPU instructions that are not properly emulated. The success of this approach motivated later works~\cite{fistful,kemufuzzer} to automate the process of generating red-pills. Similar techniques propose the exploitation of specific devices or registry keys, memory patterns or parallel running processes of known VM vendors (\eg VMWare, VirtualBox)~\cite{vmware, vbox}. A more general and advanced technique is proposed in~\cite{spotless_sand}, where the authors design an empirical ML-based technique to detect emulated environments. The approach is based on several system features (DLLs, browser cookies, \etc) that are used for training an SVM classifier and detect sanboxing environments. 

These evasion techniques triggered an arms-race with malware analysts to design countermeasures which eliminate or spoof the ``signals'' that red pill techniques exploit~\cite{barecloud}. On the other hand, attackers use (trusted) crowd-sourced malware scanning services (like VirusTotal or similar online services~\cite{sandboxes}) as a testbed to measure and tune the evasiveness of their malware. Indeed, there are  cases~\cite{graziano} where malware authors abused such services for testing their evasion mechanisms before distributing their malicious software to people.\alnote{I think here, we need to say why we need another evasion technique or better position our technique respect to the others that already exists, something like we are more agnostic, we do not depend on the specific characteristic of the software implementation of the sandbox etc.}

In this paper we introduce a novel malware evasion technique 
to create an exploitable {\it timing side-channel attack} that is able to recognize whether the malware is running on an emulated environment. To this end we design an automatic tool called  \name\footnote{A disguising suite described in the book ``A Scanner Darkly'' by Philip K. Dick~\cite{darkly}} that is a three-steps pipeline framework which executes multiple Proof-of-Work~\cite{powdwork} (POW) algorithms (e.g., blockchain technology) on several hardware platforms, and applies a statistic inequality to properly estimate the amount of time
necessary to execute such algorithms on real hardware.   In the first step of the pipeline, our framework estimates a PoW threshold that is a statistical characterization of the execution time of different PoW algorithms that run on different hardware platform. This step allows the system to select some algorithm parameters (second step) that will be used along with the PoW execution for detecting the sandbox environment and finally in the last step the system will embed in the malware the PoW algorithm with the selected parameters and run a testbed on sandbox environment to evaluate the accuracy of the sandbox detection. PoW algorithms are very suitable for such a model since, once the input parameters are fixed, their execution time only depends on a machine’s available CPU and memory (e.g, side-channel timing attack).
\jetnote{The previous par needs an additional pass to better describe the technique.}
%In this paper, we present \name\footnote{A disguising suite described in the book %``A Scanner Darkly'' from Philip K. Dick~\cite{darkly}}: a novel VM-detection %approach 
%that is effective even when the malware cannot identify neither instrumentation nor %introspection artifacts 
%at run time. \name leverages \emph{stalling code}~\cite{kruegbh,lastlinestall} to %create exploitable {\it timing side-channels attack} that is able to recognize %whether the malware is running on emulated environment (\eg sandbox). 

%This is achieved via off-the-shelf Proof-of-Work (PoW)~\cite{powdwork} algorithms (\eg blockchain technology) which stress the host and trigger hardware discrepancies. In particular {\it \name runs PoW algorithms and builds up a statistical model that is able to discern on which classes of hardware-machine (\eg real or simulated) the algorithm is running on}. 
%MV -- attempted at merging the two above sentences since this paragraph is quite long and the concept was, imho, quite similar 

%This is achieved combining off-the-shelf Proof-of-Work %(PoW)~\cite{powdwork} algorithms (\eg blockchain technology) with a %statistical model that is able to discern on which classes of %hardware-machine (\eg real or simulated) the algorithm is running %on. PoW algorithms are very suitable for such a model since, once %the input parameters are fixed, their execution time only depends on %a machine's available CPU and memory. %specific hardware machine %resources: CPU and memory usage. 
A key advantage of the evasion technique deployed by \name is that it relies on benign PoW implementations and thus it does not raise suspicion to automated malware sandboxes. Moreover, current techniques aimed at spoofing the virtualization signals present in contemporary sandboxes cannot act as countermeasures against the timing side-channels that \name exploits.

To asses the feasibility and effectiveness of \name,
%three-steps pipeline framework,
we wrote a malware PoC that implements some standard ransomware activities (e.g., scanning and encryption of files). The sample also embeds a PoW algorithm with a configuration chosen by \name. To select the appropriate PoW parameters, we ran our framework on three different hardware platforms: a low-end (Raspberry Pi 3), a medium-end (Dual Intel Xeon), and a high-end (Intel i9) machine with two different OSes (Linux Ubuntu 18.1 and Windows 10). We assumed two operational settings CPU-wise, idle and busy, to estimate a threshold that could distinguish a real hardware platform from a sandbox emulated environment. The results show that our malware sample is able to successfully evade the real sandboxes that recognize it as a benign sample.
\jetnote{Missed: which sandboxes was this tested against?}

%To asses the feasibility and effectiveness of \name, we compare %three different PoW algorithms and we implement a proof of %concept of our approach using Argon2 PoW %implementation~\cite{argon2, poc}. We integrate our prototype %into a real %malware sample (\eg 
%ransomware which delivers its malicious payload only if the %probability of running in a sandbox is low enough. We evaluate %the effectiveness of our approach on several physical and %virtual machines (Intel Core i9, Raspberry Pi, VirtualBox, %JoeSandbox and VirusTotal). Our evaluation results demonstrate %that in the best case our technique can guess the sandbox %environment in \powTimeSec with \accuracy accuracy.

\noindent{\bf Contributions.} The contributions of this paper can be summarized in the following: 

\begin{enumerate}
    \item We design \name, an automatic three-steps pipeline framework which executes multiple PoW algorithms on several hardware platforms, and applies a statistical model to properly distinguish between the real hardware platform and the emulated ones. To increase the awareness of the community we release the source code of our system \footnote{https://github.com/Raid2020Submission/Submission63}.
    
    %\item We compare the performance of 3 different Proof-of-Work algorithms on different hardware platforms and operating systems.
    
    %\item We implement a proof of concept of our approach that %utilizes the Argon2 algorithm which we integrate %our proof of concept 
    %into a real ransomware.% sample. 

    \item We evaluate the effectiveness of \name by running our prototype on executing the PoW configuration on three different hardware platforms: Raspberry Pi 3, Dual Intel Xeon, and Intel i9 machines with two different OSes Linux Ubuntu 18.1 and Windows 10 and assuming two state conditions:  idle and busy (CPU-wise). Results show the effectiveness of our method.
    
    %Our results show that \name can detect a sandbox with  \accuracy of %accuracy with an execution time of \powTimeSec.
    
    \item We perform a security analysis of our tool and we discuss limitations and potential countermeasures of our systems that could improve the defensive approach against such evasion technique. Moreover, we show how our technique can be applied in new fingerprint contexts.
\end{enumerate}


==> old/old-04_approach.tex <==
\begin{figure*}[th]
\centering
    \includegraphics[scale=.65]{"figs/System-Design.pdf"}
    \caption{Experiment Design - 1. Ansible playbook start - 2. Execution of three PoW algorithms (Argon2, Catena, YesCrypt) on different HW platforms - 3. Bounding of threshold for PoW execution to evade sandboxes - 4. Compilation and Test }
\label{fig:arch}
\end{figure*}
%MV -- compress the figure by removing all that whitespace. 

%\section{Implementation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Evading Sandboxes with \name}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This section describes \name design and implementation.
\name is a pipeline which executes at least three different PoW algorithms, on several hardware platforms, and applies the Chebyshev~\cite{chebychev} inequality to estimate properly the amount of time necessary to execute the PoW on real hardware. \mvnote{Before reaching here, the reader is kinda confused of what \name is. Is it an evasion mechanism, is it a testbed, is it an evasive malware? We need to somehow unify the writing.} \anote{it is not a malware, is it an automated tool to evade malware sandboxes, and it works end to end from threshold calculation to malware production, we changed title also because of that reason, I rephrased a bit also}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{PoW Threshold Estimation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We start by describing the tool we built to statistically estimate PoW thresholds, \ie quantify the execution times of different PoW runs on real hardware. We have chosen three of the finalists algorithms of the password hashing competition PHC~\cite{phc} for our case. In particular we have selected, Argon2 (the winner), Catena and Yescrypt. %The choice of the last two is mostly due to their good coding practices %which eased the integration in \name.

A single run of this tool involves the execution of the three different PoW algorithms  multiple times with different input parameters. %, has already explained in Section~\ref{sec:background}.
The repetition of the executions is necessary to obtain statistical meaning and significance. In a nutshell, the parameters of the algorithm allow to select the amount of memory, parallelism and complexity of the PoW. Our selection was based on common configuration of COTS hardware devices, with respect to cores, memory and CPU. However, not all the selected algorithms have these parameters available for tuning and in some cases their tuning is more coarse grained~\cite{catena}.
Next, we benchmarked \name over three hardware platforms representative of high-end, medium-end, and low-end platforms. Our high-end hardware is a desktop equipped with an Intel(R) Core(TM) i9-9900X CPU @ 3.50GHz with 10 physical cores and 20 threads equipped with an PCI-e M2 512GB disk, 32 GB of fast access RAM.
Our medium-end is a workstation equipped with a Dual Intel(R) Xeon(R) CPU E5-2643 0 @ 3.30GHz with 16 physical cores and 64GB of RAM. Finally our low-end device is a RaspberryPi3 which comes equipped with a quad core ARMv7 Processor rev 4 (v7l) and 1GB of RAM.
The idea is to produce an equal number of samples per hardware platform (300) and apply the Bienaymé–Chebyshev inequality~\cite{chebychev}%  this inequality allows to establish how much of the sample population of unknown statistical distribution is contained within a distance from the mean $\mu$.
%To be more accurate the results of the Bienaymé–Chebyshev inequality 
, which shows the percentage of the population contained between K times $\sigma$ from the mean $\mu$.

The formula $Pr(|X - \mu| \geq k\sigma) \leq \frac{1}{k^2}$ allows to select a threshold $T$ (e.g., execution time) which for \name's experimental evaluation can encompass up to 99.1\% of the sample population, see Table~\ref{tab:catena}. For our evaluation we have selected Argon2i~\cite{argon2, argon2rfc} which guarantees a 98.3\% sample population coverage.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Malware Integration.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Once \name completes the tests, it automatically calculates the threshold to evade detection based on the hardware platforms used to build its model. Our Malware PoC is written in VC++ for Windows 10 and in C++ for Linux and is roughly~150 LoC. It implements a simple ransomware which scans the entire hard drive and encrypts all its files. The idea is that the malicious behaviour is exposed only if the Argon2 PoW will be executed at least T times before a timer expires. We leverage also the Boost libraries~\cite{boost} to ease the OS interaction and build a single statically-linked executable. We selected Argon2 because from our experiments it emerges that in only ten seconds it is possible to evince whether the platform on which the executable is running is real hardware or an instrumented VM. The complete compilation step is automated as an Ansible~\cite{ansible} playbook and clang~\cite{clang}, this pipeline installs the Ansible scripts runs the tests and starts to compile the malware binary for multiple platforms automatically.

==> old/old-06_evaluation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Evaluation}
\label{sec:eval}
%%%%%%%%%%%%%%%%%%%%%%%%%
In this section, we leverage \name to evaluate the effectiveness of associating a PoW with  evasive malware. We start by empirically quantifying the execution time of popular PoWs on a spectrum of devices. Next, we built an actual ransomware which leverages the execution time of Argon2i (the PoW we have chosen, see Section~\ref{sec:background}) as an evasion mechanism, and show its effectiveness when tested on JoeSandbox~\cite{joesandbox},  Hybrid-Analysis~\cite{hanalysis}, and VirusTotal~\cite{virustotal}. 
%we have tested extensively three PoW algorithms and established solid statistical bounds to evade behavioural malware sandbox in a methodical and repeatable way.

For each PoW currently supported by \name, we have selected different configurations with respect to memory footprint, parallelism and algorithm internal iterations. All the details are in Tables~\ref{tab:argon},~\ref{tab:catena},~\ref{tab:yescrypt}. Argon2i and Yescrypt have similar parameters, like memory, number of threads, blocks, while Catena's only parameter is a graph size which grows in memory and will make its computation harder %with respect to the graph size.
as the graph size increases. 

We execute each PoW configuration on the low-end, medium-end, and high-end machines available to \name. For starters, we execute each PoW configuration for about 24 hours on each machine under optimal conditions on Linux Ubuntu 18.04.3, \ie no additional load present on the machines. 
%If additional load on the machine were considered, PoW algorithm could %perform less than usual and consequently this would just lower the %upper bound. In any case the lower bound of the Windows machine that %runs PoW algorithm in not  optimal conditions is still different in %execution time as showed in Table~\ref{tab:malhw2}. %Such lower bound is quite hard to accomplish since the difference in %terms of PoW cycles between the sandbox with the other machines is %quite hi. In this case the malware could test the PoW estimation in %different random time windows to avoid the load and detect the correct %hardware machine computation power. 
%Though, results show that to perform worse or equal than a sandbox you probably %need to use one of them and overload it. %according to an estimation performed %in optimal conditions. 
Table~\ref{tab:hw_totals} shows that, over 24 hours, both the high and medium-end platforms completed 9,000 executions of each PoW configuration (9 in total) on each platform. In comparison, the low-end platform (RaspBerry Pi 3) only completed 300 executions. The same algorithms perform worse on the same machine on Windows 10 in dual boot configuration. To validate our results on this worst case we perform an experiment where we run our malware that embeds PoW algorithm on Windows 10 machine in not optimal condition (\eg CPU-Z), see the results in Table~\ref{tab:malhw2}. Even in this worst case the Windows machine performs better than any sandboxes in terms of power execution time, Table~\ref{tab:malsand}.


%Hence, to establish a good upper bound we have selected the best %platform \ie Linux in terms of results.

%These results establish our basis to extrapolate statistical bounds on how much time $T$ is needed to detect a sandbox environment, with respect to the number of PoW that can be executed during $T$.


%In Tables~\ref{tab:argon},\ref{tab:catena},\ref{tab:yescrypt} we show the results of an unknown statistical distribution of 900 samples for the three platform. The results of the Bienaymé–Chebyshev inequality shows the percentage of the population contained between K times $\sigma$ from the mean $\mu$, according to Bienaymé–Chebyshev~\cite{chebychev} inequality $Pr(|X - \mu| \geq k\sigma) \leq \frac{1}{k^2}$.

Next, we aim at statistically investigate each PoW execution times distribution  obtained across our platforms. To do so, we leverage the Bienaymé–Chebyshev inequality. To balance equally sized data-sets, we sampled 300 random executions (\ie the total number of executions that were possible on the low-end platform) from the 9,000 executions available from both the medium and high-end platforms.  %results of the other two platforms 300 random results to obtain a uniform sample size for the three platforms.
Tables~\ref{tab:argon},~\ref{tab:catena},~\ref{tab:yescrypt} show for each PoW and configuration, several statistics (min, max, $\sigma$, and $K$, Chebyshev inequality) computed over an unknown statistical distribution of 900 execution times obtained across the three platform. The results of Chebyshev inequality show the effectiveness of the idea behind \name. With different execution parameters we were able to detect each platform with high accuracy (98\%, on average), independently of whether we are consider low-end, medium-end, or high-end hardware. %the real hardware machine architecture population represent by low-end medium-end and high-end platform.   

%Since within a small time frame it is possible to discern on which %hardware platform the PoW was executed. 
%~\mvnote{the last sentence does not read well, but was not sure how to %fix.}\anote{fixed, take a look}

Table~\ref{tab:malhw1}, summarizes the results of running \name's automated malware implementation on both Microsoft Windows 10 and Linux Ubuntu 18.04.3. We consider both the 32 and 64 bit configurations, and optimal conditions. We have included the Argon2i PoW in our PoC ransomware~\cite{ransomware}. The idea is, since for Argon2i the minimum execution time of one run of the algorithm (see Table~\ref{tab:argon} second line) on the Intel i9 is 0.2 seconds and the maximum is 9.28 under optimal conditions. \anote{@matteo check last sentence} The malware should be able to execute 50 execution of the PoW in 10 seconds. As we can evince from Table~\ref{tab:malhw1} the results are way below the expectancy on Windows 10 64bits, operated in optimal conditions. The malware PoC is able to perform only on average 28.3 executions of the proof during 10 seconds. The Linux operating system remains a point of reference because its execution times are better and hence it provides a better upper bound for \name's implementation. ~\mvnote{is this related to the impact of non being under optimal conditions? Instead of present like this, should we first remove that assumption, show this result, and then move to the next step?}\anote{this is related to the operating system, both were in idle state, it's just that windows does worse, I reorganized a bit the text}

The above results suggest us to set the evasive condition to trigger after $T=10$ seconds and check if at least $x$ number of the PoW have been completed. We have submitted different variants of the sample to different sandboxes and the results are disheartening, none of the sandbox is able to execute more than 1 cycle of the PoW, leaving a huge space of improvements of such environments.
Table~\ref{tab:malsand}, shows the results of our malware executions on sandboxes, which are normally Windows based. Which give complete results of behavioural analysis. Our malware PoC is not packed, and hence, some of the behaviour is visible through exported functions. Even though none of the samples was flagged as malicious.
The most interesting lines of Table~\ref{tab:malsand}, are the ones were we test the sandbox to perform better than a native Intel i9 and extend their time of execution to the available maximum (if possible) and double the timeout \eg $T=20 x=15$.
None of the tested sandboxes was able to perform any better of a simple RaspBerry pi. Which is a very modest hardware machine. All the reports of our analysis are publicly available, including screenshots of evasive malware samples~\cite{eva1, eva2, eva3, eva4, eva5, evavt, evavtsgamo}. While the report of same sample analyzed without evasive measure is available here~\cite{noteva, mal_vt}. It has to be noted that VirusTotal's sandbox report is not very detailed as JoeSandbox, but they both show the hard drive scan (Ransomware behaviour). Also, in Table~\ref{tab:malsand} the number of PoW executed is visible only if a screenshot of the sandbox is available. Also, with respect to the sandbox execution timeout. Both available only on JoeSandbox.
\begin{center}
\begin{table}
\caption{Full execution of 3 PoW Macro-Behchmark Results (Linux Ubuntu) }
\label{tab:hw_totals}
\centering
\begin{tabular}{|r|r|l|}
\hline
 \# Runs &  Total (hours) &  Platform\\
\hline
9,000 & 22.33 & Intel i9-9900X 3.50GHz \\
\hline
9,000 & 29.47 & Dual Intel Xeon E5-2643 3.30GHz \\
\hline
300 & 24.59 & RaspBerry Pi 3 \\
\hline
\end{tabular}
\end{table}

\begin{table*}
             \caption{Results for Argon2i Algorithm (Linux Ubuntu)}
             \label{tab:argon}
             \centering
\begin{tabular}{|r|l|r|r|r|r|r|r|c|}
\hline
 Threads & Internal Iterations & Memory & Min &  Max &  Sigma &  Mean &    K &  Chebyshev\\
\hline
 1 & 10 & 1024 KiB & 0.01 & 0.70 &  0.09 &  0.02 & 7.89 & 98.39\% \\
 \hline
 8 & 100 & 4096 KiB & 0.20 & 9.28 &  1.09 & 0.48 & 8.09 & 98.34\% \\ 
 \hline
 16 & 500 & 8192 KiB &  2.03 & 88.80 &  10.68 &  3.91 & 7.95 & 98.42\% \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\caption{Results for Catena Algorithm (Linux Ubuntu)}
\label{tab:catena}
\centering
\begin{tabular}{|c|r|r|r|r|c|c|}
\hline
 Garlic Graph Size & Min &  Max &  Sigma &  Mean &  K & Chebyshev \\
\hline
15 & 0.12 & 5.35 &   0.51 &  0.21 & 9.99 &          99.00\% \\
\hline
18 & 1.13 & 35.61 &   4.25 &  1.88 & 7.94 &          98.41\% \\
\hline
20 & 5.11 & 165.57 &  19.03 &  8.28 & 8.26 &          98.54\% \\
\hline
\end{tabular}
\end{table*}

\begin{table*}
\caption{Results for Yescrypt Algorithm (Linux Ubuntu)}
\label{tab:yescrypt}
\centering
\begin{tabular}{|r|r|r|r|r|r|r|c|c|}
\hline
 Threads & Blocks & Block Size & Min &  Max &  Sigma &  Mean &    K &  Chebyshev \\
\hline
1 & 1024 & 8KB & 0.00 & 0.02 &   0.00 &  0.01 & 6.14 &  97.35\% \\
\hline
8 & 2048 & 32KB & 0.03 & 0.56 &   0.05 &  0.05 & 10.52 & 99.10\% \\
\hline
16 & 4096 & 64KB & 0.08 & 5.00 &   0.51 &  0.19 & 9.39 & 98.87\% \\
\hline
\end{tabular}
\end{table*}
\end{center}


\begin{table*}
\caption{Malware Execution Results on Hardware (Idle) }
\label{tab:malhw1}
\centering
\begin{tabular}{|r|r|c|c|c|c|c}
\hline
Machine & Timeout & $\mu$ of \# PoW Win32 & $\mu$ of \# PoW Win64 & $\mu$ of \# PoW Linux32 & $\mu$ of \# PoW Linux64 \\
\hline
Intel i9 & 10sec & 17.5 & 28.3 & 33.2 & 48.2\\
\hline
Intel i7 & 10sec & 11.2  & 17.2 & 23.3 & 38.1\\ 
\hline
Dual Xeon & 10sec & 10.1  & 15.3 & 20.2 & 44.2\\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\caption{Malware Execution Results on Hardware (Busy with CPU-Z on Windows)}
\label{tab:malhw2}
\centering
\begin{tabular}{|r|r|c|c|c|c|c}
\hline
Machine & Timeout & $\mu$ of \# PoW Win32 & $\mu$ of \# PoW Win64\\
\hline
Intel i9 & 10sec & 15.5 & 23.5\\
\hline
Intel i7 & 10sec & 9.2  & 15.1\\ 
\hline
Dual Xeon & 10sec & 12.2 & 13.4 \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\caption{Malware Execution Results on Sandboxes}
\label{tab:malsand}
\centering
\begin{tabular}{|r|r|c|c|c|c|}
\hline
Sandbox & Evasion Timeout & PoW Check condition &\# of PoW executed & Execution Timeout & Notes\\
\hline
JoeSandbox & $10 secs$ & 50 & 1 & 120 & Clean\\
\hline
JoeSandbox & $15 secs$ & 45 & 1 & 180 & Clean\\
\hline
JoeSandbox & $20 secs$ & 40 & 1 & 240 & Clean\\
\hline
JoeSandbox & $20 secs$ & 15 & 1 & 500 & Clean\\
\hline
Hybrid-Analysis & $20 secs$ & 15 & 0 & Not available & Clean\\
\hline
VirusTotal & $20 secs$ & 45 & Not available & Not available & Clean\\
\hline
VirusTotal & $20 secs$ & 15 & Not available & Not available & Clean\\
\hline
\end{tabular}
\end{table*}


==> old/old-11_discussion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Security Analysis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The previous section demonstrates that a \name(ed) malware successfully evades popular sandbox environments. This is achieved by associating a PoW (Argon2d) with the malware, whose downside is an increase in both CPU and memory consumption. Figure~\ref{fig:cpueva} and~\ref{fig:mem_footprint}  compare, respectively,  CPU and memory utilization of our malware (red line) with \texttt{connhost.exe} (Console Windows Host) as reported by XXX. With respect to the CPU usage, the PoW associated with our malware causes an (expected) 100\% utilization for the whole duration of the PoW ($T$). With respect to  memory utilization, our malware only require about 17~MB versus, for instance, 7~MB that utilizes a sample system process like \texttt{connhost.exe}.


\begin{figure}[t]
\centering
    \tcbox[top=0pt,left=0pt,right=0pt,bottom=0pt]{{\includegraphics[scale=.45]{"figs/cpu_evader.png"}}}
    \caption{CPU Consumption of Malware PoC (Argon2d) Malware:red line connhost.exe:green line }
\label{fig:cpueva}
\end{figure}


\begin{figure}[t]
\centering
    \tcbox[top=0pt,left=0pt,right=0pt,bottom=0pt]{{\includegraphics[scale=.45]{"figs/evader_mem.png"}}}
    \caption{Memory Consumption of Malware PoC (Argon2d) Malware:red line connhost.exe:green line}
\label{fig:mem_footprint}
\end{figure}

To further investigate the impact of the above increase in CPU and memory usage of   gather 


We have tested also benign programs which are, surprisingly flagged as suspicious, while our malware is flagged as clean. In Figure~\ref{fig:cpu_z} we show the execution of the CPU-Z utility~\cite{cpuz} to fingerprint and test CPUs. This is clearly flagged as a suspicious program especially because of its CPU consumption and the multiple submission the sample has had~\cite{cpuz_eva}.

\begin{figure}[th]
\centering
    \tcbox[top=0pt,left=0pt,right=0pt,bottom=0pt]{{\includegraphics[scale=.321]{"figs/cpu_z.png"}}}
    \caption{CPU Consumption of CPU-Z Utility, CPU-Z:red line connhost.exe:green line}
\label{fig:cpu_z}
\end{figure}

We have further tested countermeasures to reduce the CPU usage of our PoC ransomware. First we have reduced the PoW execution and the timeout $T$ to 3 seconds and obtained less CPU drain, with a peak of 80\% as it is possible to see in Figure~\ref{fig:evader_ant}. The complete report is available here~\cite{mal_ant1}. This reduces the suspiciousness of the sample but, using such a small $T = 3$ seconds, reduces also the margin to evade the sandbox and hence easily detectable.

\begin{figure}[th]
\centering
    \tcbox[top=0pt,left=0pt,right=0pt,bottom=0pt]{{\includegraphics[scale=.321]{"figs/evader_ant.png"}}}
    \caption{CPU Consumption of Malware PoC $T=3$ seconds, Malware:red line connhost.exe:green line}
\label{fig:evader_ant}
\end{figure}

As another approach we have tried is make our PoW to go low-and-slow, by setting $T = 60$ seconds and a sleep of $.5$ seconds between each execution of the PoW. Figure~\ref{fig:evader_ant2} yet, shows a very high CPU usage, which means that to obtain a smoother curve the sleep has to last more time. However this would transform our PoW approach into an effective stalling code solution, which sleeps. The report is available here~\cite{mal_ant2}. Moreover since the plots are coming directly from the sandbox the sleeping time could be not sufficient with respect to their measurement sampling rate of CPU drain.


\begin{figure}[th]
\centering
    \tcbox[top=0pt,left=0pt,right=0pt,bottom=0pt]{{\includegraphics[scale=.321]{"figs/evader_ant2.png"}}}
    \caption{CPU Consumption of Malware PoC $T=60$ seconds, Malware:red line connhost.exe:green line}
\label{fig:evader_ant2}
\end{figure}

We also compare the behavioural maps of our malware PoC vs CPU-Z in Figures~\ref{fig:subpoc} and ~\ref{fig:subcpuz} and as it is possible to see, CPU-Z is clearly shown as a false positive from the sandbox. Indeed, CPU-Z is a more complex software respect to a simple ransomware that scans the hard drive and encrypts every file. Though, it does not have anything malicious in it.

\begin{figure}[ht]
\centering
\begin{subfigure}
  \centering
  \includegraphics[scale=.3]{figs/evader.png}
  \caption{Malware PoC Behavioural Map}
  \label{fig:subpoc}
\end{subfigure}

\begin{figure}
    \centering
    \includegraphics[scale=.3]{figs/naked.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}



%
\begin{subfigure}
  \centering
  \includegraphics[scale=.3]{figs/benign.png}
  \caption{CPU-Z Behavioural Map}
  \label{fig:subcpuz}
\end{subfigure}
\end{figure}

Another important aspect to underline, of Figures~\ref{fig:subpoc} and~\ref{fig:subcpuz} is that our Malware PoC is neither packed nor stripped, and hence some of its functionality \ie exported functions, linked libraries, and function names are visible through basic static analysis as noted before. With some extra effort our zero-day malware would be undetectable for a good amount of time and its behavioural map would look even greener. Raising the detection bar even more.

==> old/old_00_abstract.tex <==
\begin{abstract}
Malware analysis systems are one of the best weapons in the arsenal of cybersecurity companies and researchers. An integral part of such systems is a sandbox providing an instrumented and isolated environment to run unknown artefacts and observe their behavior to identify potentially malicious actions. In order to avoid detection, attackers have developed numerous techniques to make analysis harder. One class of anti-analysis attacks is based on the observation that it is not only the sandbox that monitors the behavior of the running program; the program itself can also monitor its surrounding environment to detect the presence of a sandbox and try to evade it. This is usually achieved by looking for artifacts suggesting that the execution environment is a sandbox, such as specific memory patterns, behavioral traits of certain CPU instructions (known as red pills), or parallel running processes of known Virtual Machine (VM) vendors. To mitigate this threat, sophisticated sandboxes remove or spoof these signals, thus making it harder for a malware sample to detect the emulated environment.
In this paper we devise a new evasion strategy based on Proof-of-Work (PoW) algorithms that show an asymptotic behavior, in terms of computational cost, when they run on some class of hardware platform. To this end such algorithms can be used to effectively detect virtualized environment (e.g., malware sandbox analysis). To prove the validity of this intuition, we design and implement \name: a tool that is able to automatically implement such detection strategies and embed a test evasion program into an arbitrary malware sample. Evaluation results show that the proposed detection technique can evade the most popular public sandboxes.
\end{abstract}

%The reason of using PoW implementations is that they put under heavy load physical machines and have, according to our results, higher accuracy in distinguishing machines used by legit users with respect to sandboxes, depending on their execution time. 

==> old/old_01_introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\$1.5 trillion dollars (or \$2.9 million dollars per minute)~\cite{malwarecost2018}, with predictions 
hinting at this cost to reach \$6 trillion dollars by 2021~\cite{malwareCost}. 

Due to the sheer amount of known malware samples~\cite{virushare, virustotalstats},  manual analysis neither scales nor allows to build any comprehensive threat intelligence around the detected cases (\eg malware clustering by specific behavior, family or infection campaign). To address this problem, security researchers have introduced \emph{sandboxes}~\cite{anubis}: isolated environments that automate the dynamic execution of malware and monitor its behavior under different scenarios. Sandboxes usually comprise a set of virtual machines instrumented to gather fundamental information of the malware execution, such as system calls, registry keys accessed/modified, new files created, and memory patterns. Such techniques are extensively used by antivirus companies or online scanning services (\eg VirusTotal) that analyze malware samples submitted by users. Sandboxes have also become critical for mobile app for online marketplaces~\cite{sandboxandroid}. 
%Apart from the sandbox that monitors the behavior of the malware, in %some cases, the malware itself is monitoring its environment to detect %the presence of a sandbox. So called \emph{evasie} malwares use various %sophisticated techniques to detect virtualized environments and pause %the delivery of their malicious payload. %thus evading detection. 

Sandboxing is only successful at detecting malicious behavior if it goes undetected. If a malware sample can detect the presence of a sandbox, it can simply abort the execution of any malicious payload. The \emph{red pill}~\cite{1624022,fistful,kemufuzzer} is a popular technique to detect virtualized environments by leveraging CPU instructions, registry keys, memory patterns, and other artifacts that are not correctly emulated. Regardless of the specific technique used, the above detection mechanism does not work in advanced sandboxes that can spoof the ``signals'' that red pill techniques exploit~\cite{barecloud}. This has motivated miscreants to use (trusted) crowd-sourced malware scanning services (like VirusTotal or similar online services~\cite{sandboxes}) as a testbed to measure and adjust the evasiveness of their malware programs. 
More recently, \cite{spotless_sand} proposes to use several system features (DLLs, browser cookies, \etc) to train an SVM classifier and detect sandboxing environments. Such a technique needs a training phase based on a real environment and it should exactly know which system resources need to be considered.

In this work, we introduce a new set of evasion strategies based on Proof-of-Work (PoW)~\cite{powdwork} algorithms. Our intuition lies on the fact that, like NP-class problems~\cite{npp}, the asymptotic behavior of a PoW algorithm is constant in terms of computational cost~\cite{powdwork}, \eg CPU and memory consumption. Accordingly, PoW algorithms are perfect candidates for benchmarking the capability of the hardware where they are run, revealing the absence or presence of a sandbox because of the deviation with respect to the expected measured performance.
%Moreover, current techniques aimed at spoofing the virtualization signals present in contemporary sandboxes cannot act as countermeasures against the timing side-channels that \name exploits.
A key advantage of using PoW techniques is that they are self-contained mechanisms compared to the other more fine-grained timing side-channel approaches. In fact, it does not require the access to precise timing resources for detecting the emulated environment (e.g., network or fine-grained timers). The technique is robust enough since it can detect the
emulated environment with high precision just by looking at the output of the algorithm, as we will show in the experiments.
Moreover, it relies on PoW implementations that do not raise any suspicion to automated malware sandboxes. While stalling code e.g. (infinite loops and/or sleep) are easier to detect because of CPU idleness. Fingerprinting PoW algorithm as a malware component is feasible e.g. by checking the usage of particular cryptographic instructions. Though, it can produce a huge number of false positive compared with more fine-grained ad-hoc side-channel techniques~\cite{10.1145/2818000.2818030}. This because PoW algorithms can be part of a legit application.
Using the above idea, we built \name,\footnote{A disguising suite described in the book ``A Scanner Darkly'' by Philip K. Dick~\cite{darkly}} a framework to automatically create, inject, and evaluate PoW-based evasion strategies in arbitrary programs. \name operates as a three-steps pipeline. During the fist step, multiple PoW algorithms are tested across different hardware platforms (Raspberry Pi 3, Dual Intel Xeon, Intel i9), operating systems (Linux Ubuntu 18.03 and Windows 10), and machine loads. These extensive tests are used to build a statistical characterization of each PoW execution time in each setting, using the Bienaym\'{e}–Chebyshev inequality~\cite{chebychev} to obtain sound statistics about the expected execution time. In the next step, a miscreant can upload its malware to \name and select the evasion mechanism to be used. Finally, \name automatically evaluates the accuracy of the evasion mechanism selected, when coupled with the uploaded malware, via several tests run both on a local sandbox and on multiple on-line free-of-charge sandbox services~\cite{sandboxes}.

We empirically evaluate each step of \name's pipeline. For the PoW threshold estimation, we have tested three popular PoW algorithms
(Catena~\cite{catena}, Argon2~\cite{argon2,argon2rfc} and Yescrypt~\cite{yescrypt}) using multiple configurations. During 24 hours of testing, we find Chebyshev inequality values higher than 97\% regardless of the PoW and configuration. This confirms high determinism in the PoW execution times on real hardware, thus validating the main intuition behind this work.
We test our technique over two known ransomware families by submitting to VirusTotal several variants that include PoW-based evasion. The results demonstrate how the inclusion of this mechanism reduces the number of detections, even in the presence of other anti-analysis techniques such as code virtualization or packing.
To further analyze its impact on real-world analysis sandboxes, we wrote a  fully functional malware sample, integrated an evasion mechanism based on Argon2, and submitted it to JoeSandbox~\cite{joesandbox}, Hybrid-Analysis~\cite{hanalysis}, and VirusTotal~\cite{virustotal}). Reports from each sandbox all mark our malware as \emph{clean}, validating the effectiveness of a PoW-based evasion mechanisms. We further discuss the behavioral analysis reported by JoeSandbox for our malware, as well as potential countermeasures to this novel PoW-based evasion mechanism we have proposed.

In order to increase the reproducibility of our results and foster further research on this topic, we make the source code of our system publicly available.\footnote{\url{https://github.com/anonnymousubmission/anonymousubmission}}

%\footnote{https://github.com/Raid2020Submission/Submission121}

\paragraph{Organization.}
The rest of this paper is organized as follows. Section~\ref{sec:background} provides some background on PoW algorithms. Section~\ref{sec:framework} introduces our evasion framework, which is evaluated in Section~\ref{sec:eval} against real-world malware sandboxing services. Section~\ref{sec:analysis} discusses in detail the behavioral reports obtained from the sandboxes, and Section~\ref{sec:defences} discusses possible countermeasures. Sections~\ref{sec:related} and \ref{sec:ethics} discuss related work and ethical considerations, respectively. Finally Section~\ref{sec:conclusion} concludes the paper summarizing our main contributions and discussing future work.

==> old/old_09_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
\name represents one further step in the evolution of evasion techniques for malware. We believe that the application of PoW as a malware evasion technique is an innovative and provocative idea, exposing a weaknesses in our current analysis platforms. In this paper, we have provided empirical evidence of how it can be used to evade real-world malware analysis sandboxes, and discussed potential countermeasures. Furthermore, our implementation of \name goes beyond a simple PoC, showing that injecting evasion modules can be easily automated on any arbitrary sample. We make our code and results publicly available in an attempt to increase reproducibilty and stimulate further research in this area.
%Malicious software has become very complex, and often very targeted. all the techniques that are used to evade, thwart and ultimately avoid detection are often inherited from different samples or derived from particular vulnerabilities of the specific target. However, \name shows a new generic technique that can be used maliciously to avoid detection and indirectly foster the expansion of malicious software to new unprotected victims. For this reason is very important to act and find viable countermeasures against such principled approaches which could really change the way malware is executed and exposes its behaviour. We have proposed several techniques that can help to mitigate such attack.


%Indeed, PoW is the ultimate frontier to avoid attacks to distributed systems such as %blockchain and its power has been demonstrated through the fact that transactions %cannot be replayed and crypto-coins cannot be double spent. 
%Moreover, \name goes beyond a simple PoC, showing that it can be easily automated %and expose weaknesses and limitations of malware analysis platforms, in a principled, methodical and repeatable way. 
%Moreover \name shows that is able to fingerprint a sandbox within only $10$ seconds in a %way that cannot be fixed with a simple workaround. 
%Indeed, combining \name with a good packing technology, which could be an %emulator~\cite{rotalume} or a known twist of existing packers~\cite{ugarte} can make %dynamic analysis quite hard. 

%On the other hand, as we mention as countermeasure techniques there are possibilities to %fingerprint PoW algorithms inside malware. Also enhancing sandboxes to execute crypto %operations, on which PoW are based, natively even if the virtualized environment is %instrumented can help to raise the bar. 
%In Section~\ref{sec:futures} we evaluate potential enhancements of \name and defences %against it.


%\point{Future Work}
%\label{sec:futures}
%\paragraph{Malware Automation}
%Our aim is to continue to study the phenomena that surrounds malware, its analysis, and the countermeasures that can be applied to thwart such analysis. We envision that attack-driven research is a necessary approach to demonstrate the duality of every phenomena that are in conflict. In this specific case we think that malware could in the future, thwart analysis directly trying to mine the last block of a public blockchain as some JS based malware was doing to get rewarded. In this case, the mining would serve as stalling code to evade detection. Moreover, updates to the malware evasion time can be done on the fly when the next block of the blockchain is calculated, thus automating the evasive behavior upgrade.

%\paragraph{CPU Fingerprinting}
%With a very granular source of time, given the asymptotic behavior of the PoW algorithms we believe that they may be used to fingerprint hardware platforms instead of simply distinguishing sandboxes from real hardware. The potential of this proposal is to perform such fingerprinting remotely as Sánchez-Rola~\cite{clock} did, \ie through the browser. This opens many new questions about user profiling, privacy and security. However, since the well-known micro-architectural bugs Spectre, Meltdown, and Foreshadow~\cite{spectre, meltdown, foreshadow} the timer resolution granularity of browsers, normally accessed through the $performance.now()$ JavaScript function~\cite{perfNow} has been highly reduced, so fingerprinting a specific CPU based on execution time can become a daunting task and requires a lot of time or generate many false positives.

==> old/unused_05_implementation.tex <==
\section{Implementation}
Implementation is divided in two phases, first we will describe the implementation of the testbed and its execution program. Second we will describe an implementation of a potential ransomware program which leverages PoW as an evasion measure. All the code of the implementation is available at~\cite{poc}.
\paragraph{Testbed Implementation.}
The test program has been implemented in Python3 language with approximately 100 LoC. Every experiment has been designed to last approximately a single day based on the hardware capabilities of the machines. For each PoW we have tested three different configuration which we will accurately describe in the Section~\ref{sec:evaluation}. In a nutshell the different parameters allow to select the amount of memory, parallelism and complexity of the PoW. We repeated the experiment as much as possible during approximately 24 hours to obtain meaningful statistics.
\paragraph{Malware Implementation.}
Our PoC is written in VC++ for Windows 10 and is roughly ~150 LoC. It implements an example of a ransomware, which scans the entire hard drive and encrypts all the files into it. The idea is that the malicious behaviour is exposed only if the Argon2 PoW will be executed at least T times before a timer expires. 
\label{sec:implementation}
